Goodness-of-Fit Testing for H\"older-Continuous Densities: Sharp Local Minimax Rates

We consider the goodness-of fit testing problem for H\"older smooth densities over $\mathbb{R}^d$: given $n$ iid observations with unknown density $p$ and given a known density $p_0$, we investigate how large $\rho$ should be to distinguish, with high probability, the case $p=p_0$ from the composite alternative of all H\"older-smooth densities $p$ such that $\|p-p_0\|_t \geq \rho$ where $t \in [1,2]$. The densities are assumed to be defined over $\mathbb{R}^d$ and to have H\"older smoothness parameter $\alpha>0$. In the present work, we solve the case $\alpha \leq 1$ and handle the case $\alpha>1$ using an additional technical restriction on the densities. We identify matching upper and lower bounds on the local minimax rates of testing, given explicitly in terms of $p_0$. We propose novel test statistics which we believe could be of independent interest. We also establish the first definition of an explicit cutoff $u_B$ allowing us to split $\mathbb{R}^d$ into a bulk part (defined as the subset of $\mathbb{R}^d$ where $p_0$ takes only values greater than or equal to $u_B$) and a tail part (defined as the complementary of the bulk), each part involving fundamentally different contributions to the local minimax rates of testing.

==> Proof_densities/Values_constants.tex <==
\section{Values of absolute constants}

\begin{itemize}
    \item $\cstar = $
    \item $\CbulkLB = \frac{2{\Cphi }^t}{(4\ch)^{\alpha t}} \int_{\R^d} \big(1 - \|y\| \big)_+^{\alpha t} dy$
    \item $\Ctilde = 2\frac{{\Ch}^d {\Cp}^2}{{\cp}^2 {\ch}^{4 \alpha + 2d}} \int_{\R^d}(1 - \|x\|)^\alpha dx$
    \item $\Cphi =  \Big(\frac{2}{\Ctilde} \log(1+4(1-\eta)^2) \Big)^\frac{1}{4} \land \cA \big(4 \Ch \big)^\alpha$
    \item $\ctail = 4/\sqrt{\eta}$
    \item $\CtailLB = \Big[\frac{1}{2} \cgamma \int_{\R^d} (1- \|y\|)_+^{\alpha t} dy\Big]^\frac{1}{t}$
    \item $\CL{\ref{Toute_la_case_OK_moment2}} = \Cmom \lor 12\cu $
    \item $\calpha \geq \frac{2}{1/2 - \cstar} \left(\frac{\sqrt{d}}{2} \right)^\alpha$
    \item $\cA = 4.001 \lor 2(2\sqrt{d})^\alpha$
\end{itemize}

==> contents_densities/Extension_to_non_bounded_domain.tex <==
\section{Extension to non bounded domain}

We now show how our analysis for densities on $[0,1]^d$ can be transferred to handle the case of densities on $\R^d$. By convention, we consider $\R^d$ as a cubic domain of $\R^d$. Note that any density defined over a bounded cubic domain in $\R^d$ can be modified through translation and rotation to get a density over $[0,\lambda]^d$ for some $\lambda>0$. We consider $d$ and $t$ as being fixed. Introduce, for any cubic domain $\Omega' \subset \R^d$:
\begin{align}
    %\forall a < b: \mathcal{P}_{a,b}(\alpha,L,\cstar) &= \left\{p\text{  density over } [a,b]^d ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $[a,b]^d$} \right\}, \label{def_P_ab}\\
     \mathcal{P}_{\Omega'}(\alpha,L,\cstar) &= \left\{p\text{  density over } \Omega' ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $\Omega'$} \right\}, \label{def_P_cubic}
\end{align}
If $\Omega'$ is of the form $[0,\lambda]^d$ for $\lambda>0$, we denote for simplicity $\mathcal{P}_{\Omega'}(\alpha,L,\cstar)$ by $\mathcal{P}_\lambda(\alpha,L,\cstar)$.
%$\forall \lambda>0: \mathcal{P}_\lambda(\alpha,L,\cstar) &= \left\{p\text{  density over } [0,\lambda]^d ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $[0,\lambda]^d$} \right\}, \label{def_P_H}\\$
Fix $\lambda_1, \lambda_2>0$ and $\lambda=\lambda_1/\lambda_2$. Define the rescaling operator:
\begin{equation}\label{rescaling_operator}
    \Phi_{\lambda_1,\lambda_2}: \left\{ \begin{array}{ccc}
        \mathcal{P}_{\lambda_1}(\alpha,L,\cstar) & \longrightarrow & \mathcal{P}_{\lambda_2}(\alpha, L \lambda^{\alpha+d},\cstar)\\
        &&\\
        p & \mapsto & \lambda^d\, p(\lambda \, \cdot \,) 
    \end{array}\right. 
\end{equation}
where $p(\lambda \, \cdot \,) : x \mapsto p(\lambda x)$. We show in Lemma \ref{Rescaling} that $\Phi_{\lambda_1,\lambda_2}$ is the natural operator for transferring the rates over $[0,\lambda_1]^d$ to $[0,\lambda_2]^d$. For any cubic domain $\Omega' \subset \R^d$, we define $\rho_{\Omega'}^*(p_0,\alpha,L,n)$ as the minimax separation radius for the following testing problem over $\Omega'$, upon observing $X_1,\dots,X_n$ iid with density $p \in \mathcal{P}_{\Omega'}(\alpha,L,\cstar)$ 


%For fixed $\lambda>0$ and for $p_0 \in \mathcal{P}_\lambda(\alpha,L,\cstar)$ (resp. $p_0 \in \mathcal{P}_{\R^d}(\alpha,L,\cstar)$), define $\rho_\lambda^*(p_0,\alpha,L,n)$ (resp. $\rho_{\R^d}^*(p_0,\alpha,L,n)$ ) as the minimax separation radius for the following testing problem over $[0,\lambda]^d$ (resp. $\R^d$), upon observing $X_1,\dots,X_n$ iid with density $p \in \mathcal{P}_\lambda(\alpha,L,\cstar)$ (resp. $\mathcal{P}_{\R^d}(\alpha,L,\cstar)$):
\begin{align}\label{testing_pb_lambda}
\begin{split}
    H_0~~~ &: \; p = p_0 \;\;~~~~~~\; \text{ versus }\\
    H_1^{(\Omega')}(\rho) &:\; p \in \mathcal{P}_{\Omega'}(\alpha,L', \cstar') ~ \text{ s.t. } \|p-p_0\|_t \geq \rho.
\end{split}
\end{align}
Similarly, if $\Omega'$ is of the form $[0,\lambda]^d$ for $\lambda>0$, we denote for simplicity $\rho_{\Omega'}^*(p_0,\alpha,L,n)$ by $\rho_\lambda^*(p_0,\alpha,L,n)$.
We now state the following Proposition, guaranteeing that our analysis over $[0,1]^d$ can be transferred, by homogeneity, to densities on any bounded cube $[0,\lambda]^d$ for $\lambda>0$, and by translation and rotation, to any cubic domain in $\R^d$. 

\begin{proposition}\label{transfer_rate}(Rescaling)
Let $\lambda_1, \lambda_2>0$ and $\lambda = \lambda_1/\lambda_2$ and let $p_0 \in \mathcal{P}_{\lambda_1}(\alpha,\, L,\,\cstar)$. It holds
$$ \rho_{\lambda_2}^*\left(\Phi_{\lambda_1,\lambda_2}(p_0),\, \alpha,\, L\lambda^{\alpha+d},\, n\right) = \lambda^{\frac{d}{t}-d}\,\rho_{\lambda_1}^*\left(p_0, \alpha, L, n \right).$$
\end{proposition}

We can now analyze the unbounded case. The following Proposition states that the unbounded case can be deduced from the bounded case by restricting the density to a sufficiently large bounded cubic domain $\Omega'$ (in the sense that the total mass of $p_0$ outside $\Omega'$ is at most $O(1/n)$.) Moreover, an optimal test on $\R^d$ can be obtained by combining any optimal test on $\Omega'$ with the test rejecting $H_0$ whenever at least one of the observations $(X_i)_i$ belongs to $\R^d \setminus \Omega'$.\\

Let $p_0 \in \mathcal{P}_{\R^d}(\alpha,L,\cstar)$. Set $\lambda>0$ such that $V:= \int_{[-\lambda,\lambda]^d}p_0 \geq 1- \frac{\cRd}{n}$ for some  constant $\cRd$ sufficiently small. Define $\Omega' = [-\lambda,\lambda]^d$ and $$\barpzero : \Omega' \longrightarrow \R_+; ~ x\mapsto \frac{1}{V}p_0(x).$$ 
For all $\rho>0$, define
\begin{equation}\label{def_P_omega_rho}
    \mathcal{P}_{\Omega'}(\rho) = \{p \in \mathcal{P}_{\Omega'}(\alpha, L,\cstar) : \|p-\barpzero\|_t \geq \rho\}.
\end{equation}
For any test $\psi$ and all $\rho>0$, define the risk of $\psi$ with radius $\rho$ on $\Omega'$:
\begin{equation}\label{risk_Omega'}
    R_{\Omega'}(\psi, \rho) =  \mathbb{P}_{\barpzero}(\psi=0) + \sup_{p \in \mathcal{P}_{\Omega'}(\rho)} \mathbb{P}_p(\psi=1) .
\end{equation}

\begin{proposition}\label{unbounded_case}(Unbounded case)
It holds: $$\rho_{\R^d}^*(p_0, L,n) \asymp \rho_{\Omega'}^*(\barpzero, L,n).$$
Moreover, if $\barpsistar$ is a test satisfying $R_{\Omega'}(\barpsistar, C\rho_{\Omega'}^*(\barpzero, L,n)) \leq \frac{\eta}{2}$ for some  constant $C$ sufficiently large, then, for $\psi^* := \barpsistar \lor \mathbb{1}\left\{\bigvee\limits_{i=1}^n (X_i \notin \Omega')\right\}$, we have: $R_{\R^d}(\barpsistar, C'\rho_{\Omega'}^*(\barpzero, L,n)) \leq \eta$ for some  constant $C'$ sufficiently large.
%Moreover, for all $\rho>0$ define $\mathcal{P}_{\Omega'}(\rho) = \{p \in \mathcal{P}_{\Omega'}(\alpha, L,) : \|p-\barpzero\|_t \geq \rho\}$. 

\end{proposition}



==> contents_densities/Poubelle.tex <==
%Ancienne justif du Lemme \ref{cov_close}

This implies $p_0(x) \leq p_0(y)$. Note that by Lemma \ref{const_balls}, we have 
\begin{equation}\label{sup_ball_p}
    \sup_{z \in B(x,h(x))}p_0(z) \leq \big(1 + \frac{\cstar}{\cA}\big)p_0(x)
\end{equation}
%\begin{equation}\label{inf_ball_h}
%    \inf_{z \in B(x,h(x))}h(z) \geq (1 - %\cstar)^\frac{2}{(4-t)\alpha + d} h(x)
%\end{equation}
Set $\CKprime = \int_{\R^d} K^2$, then:
\begin{align}
    &\left|\text{cov}\left(K_{h(x)}(x-X),K_{h(y)}(y-X)\right)\right|  \leq \sqrt{\V\left(K_{h(x)}(x-X)\right)\V\left(K_{h(y)}(y-X)\right)} \nonumber \\
    & \leq  \sqrt{\CKprime\frac{\sup_{z \in B(x,h(x))}p_0(z) }{h(x)^d }} \sqrt{\CKprime\frac{\sup_{w \in B(y,h(y))}p_0(w)}{h(y)^d}}~~~~ \text{ by \cite{tsybakov2008introduction}, Proposition 1.1}\nonumber\\
    & \leq \CKprime \frac{\Cp p_0(y)}{ h(x)^d }\nonumber \\
    & \leq \CKprime \; \frac{\Cp}{ h(x)^d } \; \frac{p_0(x)}{\cp} =: \; \Cclose \frac{p_0(x)}{h(x)^d} \label{xy_far}
\end{align}

In the last line, we use Lemma \ref{const_balls} to get $p_0(x) \geq \cp p_0(y)$ since $x \in B(y, h(y))$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Lemme pour borne inf bulk


We will need the following lemma:
\begin{lemma}\label{int_phij2_p0}
There exist two absolute constants $\cphi, \Cphi >0$ such that for all $j=1, \dots, N$:
$$\int_\Omega \frac{\phi_j^2}{p_0} = \Cphi L h$$
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Truc avec U

Let $\cu = $ \ju{compléter} and define $U \in \{1, \dots, M\}$ as
\begin{equation}\label{def_U}
    U = \min \Big\{j \in \{1,M\}: n^2 \big(\int_{C_j} p_0 \big) \sum_{l\geq j} \int_{C_l} p_0 \leq \cu \Big\}.
\end{equation}

We recall that the cells $(C_j)_j$ are sorted by decreasing order of mass under $H_0$. Define $D(U) = \cup_{j \geq U} C_j$. For $j \geq U$ we define 
\begin{equation}\label{def_pi}
    \bar \pi = \frac{\cu}{ n^2\int_{D(U)} p_0} \text{ and } \pi_j = \frac{1}{\bar \pi} \int_{C_j} p_0.
\end{equation}
\ju{Donner la valeur de $\cu$.}

The index $U$ has no further meaning than to guarantee for all $j\geq U$ : $\pi_j \in [0,\cu]$. In particular, $\pi_j$ is a Bernoulli parameter. We define the family of independent Bernoulli random variables $b_j \sim Ber(\pi_j)$ for all $j \geq U$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ancien prior avec lambda uniforme

In this case, we set a sparse prior. We once again use the partition of the tail $\{C_1, \dots, C_M\}$ defined above. Set
\begin{equation}\label{def_lambda}
    \lambda = \frac{1}{M}\Big( n  \int_{\B^c} p_0\Big)^2
\end{equation}
\begin{lemma}\label{lambda_leq_1}
It holds $\lambda \leq 1$.
\end{lemma}
Lemma \ref{lambda_leq_1} allows us to define the family of $iid$ Bernoulli random variables $\forall j=1, \dots, M: b_j \overset{iid}{\sim} Ber(\lambda)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ancien lemme reliant U et I + concentration avec le prior tail avec $\pi_i$ pas unif


Then by Lemma \ref{I_and_U}, we are necessarily in the case $\int_{D(U)} p_0 \geq \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0$. Otherwise, if $\int_{D(U)} p_0 < \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0$, then we would still have by Lemma \ref{I_and_U}:
\begin{align*}
    \int_{\mathcal{T}(\uI)} p_0 &\leq \int_{D(U)} p_0 + \frac{\sqrt{\cI}}{n}\\
    & < \frac{1}{3} \int_{\mathcal{T}(\uI)} p_0 + \frac{\sqrt{\cI}}{n}
\end{align*} hence: $\int_{\mathcal{T}(\uI)} p_0 \leq \frac{3}{2}  \frac{\sqrt{\cI}}{n}$ which is excluded since we assume $\int_{\mathcal{T}(\uI)} p_0 \geq \frac{1}{n}$.\\




\subsection{Technical results}

\begin{lemma}\label{I_and_U} It holds : $$\int_{D(U)} p_0 + \frac{1}{n} \asymp \int_{\mathcal{T}(\uI)} p_0 + \frac{1}{n}.$$ Moreover, we either have $$\int_{D(U)} p_0 \geq \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0 ~~ \text{ or } ~~ \int_{\mathcal{T}(\uI)} p_0 \leq \int_{D(U)} p_0 + \frac{\sqrt{\cI}}{n}$$
\end{lemma}

\begin{proof}[Proof of Lemma \ref{I_and_U}]
In this proof, we will use the following notation:
$$\forall j =1, \dots, M: ~p_j:= \int_{C_j} p_0.$$
\vspace{-8mm}
\begin{align*}
     S ~~ &:=~ \sum_{j=1}^M p_j = \int_{T(\uI)} p_0 \\
     S_U ~ &:=~ \sum_{j \geq U} p_j = \int_{D(U)} p_0 \\
    S_{-U} &:=~ S - S_U\\
    h ~ & ~ = \hT(\uI)
\end{align*}
We want to prove $S + \frac{1}{n} \asymp S_U + \frac{1}{n}$ and $\big[ S_U \geq \frac{1}{3} S \text{ or } S \leq S_U + 2\frac{\sqrt{\cI}}{n} \big]$.
If $S_U \geq S/3$ then the result is clear. Assume $S_U < S/3$. Then $S_U < \frac{1}{2} S_{-U}$. Let $V \in \{1, \dots, U-1\}$, then:
\begin{align*}
    \int_{C_V} p_0^2 + \frac{1}{2} \frac{\cI}{n^2 h^d} &\geq \int_{C_V} p_0^2 + \frac{1}{2}\int_{\mathcal{T}(\uI) \setminus D(U)} p_0^2 ~~ \text{ by definition of } \uI\\
    &\\
    & \geq \frac{1}{h^d}\, p_V^2 + \frac{1}{2} \sum_{j < U} \frac{1}{h^d} \, p_j^2 ~~ \text{ by the Cauchy-Schwarz inequality}\\
    & > \frac{p_{U-1}}{h^d} \big(p_{U-1} + \sum_{j \geq U} p_j\big) ~~ \text{ since } S_U < \frac{1}{2} S_{-U}\\
    & > \frac{\cu}{n^2h^d} ~~ \text{ by definition of }U.
\end{align*}
Therefore, it holds for all $V < U$:
\begin{equation}\label{CV}
    \int_{C_V} p_0^2 > \frac{\cu - \cI/2}{n^2 h^d} \geq \frac{\cI}{2n^2 h^d}
\end{equation}
Moreover by definition of $\uI$:
\begin{align*}
    \frac{\cI}{n^2h^d} \geq \int_{\mathcal{T}(\uI) \setminus D(U)} p_0^2 = \sum_{j<U} \int_{C_j} p_0^2 > (U-1)\frac{\cI}{2n^2h^d} ~~\text{ by  \eqref{CV}}
\end{align*}
Therefore: $U \leq 2$ so $U=2$ since otherwise we would not have $S_U < S/3$. Then
\begin{align*}
    S = p_1 + S_U \leq \sqrt{h^d \int_{C_1}p_0^2} + S_U \leq \frac{\sqrt{\cI}}{n} + S_U
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ancien terme II H0

\hfill

We first prove that $\int\omega(x)p_0(x)^2 dx \gtrsim t_n$. \ju{Gros problème}
\begin{align}
    \int\omega(x)p_0(x)^2 dx &= \int p_0^\frac{2\alpha t - 4\alpha}{(4-t)\alpha + d}\frac{1}{\left(n^2L^2\I\right)^\frac{d}{4\alpha+d}}\nonumber\\
    & \geq \frac{1}{L^\frac{2d}{4\alpha+d}} \I^\frac{4\alpha}{4\alpha+d}\uA^\frac{4\alpha + 2d - 2\alpha t}{4\alpha + d - \alpha t}\nonumber\\
    & \gtrsim \frac{1}{L^\frac{2d}{4\alpha+d}} \I^\frac{4\alpha}{4\alpha+d}\left[\frac{L^d}{n^{2\alpha}\I^\alpha}\right]^{\frac{1}{4\alpha+d}\frac{(4-t)\alpha + d}{(2-t)\alpha + d}\frac{4\alpha + 2d - 2\alpha t}{4\alpha + d - \alpha t}}\;\;\;\; \text{ by lemma \ref{lemma_uA}} \nonumber\\
    & = t_n\label{Exp_geq_tn}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ancienne remarque sur $\hT(\uA)$ et $\bar \hT(\uI)$


\ju{Remarque clé ? $\hT(\uI) \asymp \hT(\uA)$ sauf peut-être cas pathologique où $\int_{\widetilde{T}} p_0 \gg \int_{\mathcal{T}} p_0$. En effet: 
\begin{align*}
    \frac{1}{n^2\hT^d(\uA)} \lesssim \int_{\Tail} p_0^2 \lesssim \frac{1}{n^2 \hT(\uI)^d}
\end{align*} or clairement, $\hT(\uA) \leq \hT(\uI)$. Est-ce qu'il faudrait pas définir $\hT$ avec $\uA$ plutôt que $\uI$ ?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Truc sous H1:
\begin{align}
    \E^2\left[\hat \Delta(x) \hat \Delta(y)\right] \leq \; & 2\; \E\left[K_{h(x)}(x-X) - p_0(x)\right]^2\E\left[K_{h(y)}(y-X) - p_0(y)\right]^2 \nonumber\\ 
    & + 2\left[\frac{1}{k} \text{cov}\left(K_{h(x)}(x-X),K_{h(y)}(y-X)\right)\right]^2 \label{exp_delta2_delta2}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
    &\iint_{\B^2} \omega(x) \omega(y) \E\left[K_{h(x)}(x-X) - p_0(x)\right]^2\E\left[K_{h(y)}(y-X) - p_0(y)\right]^2 \nonumber \\
    &\leq \left[\int_\B \omega(x) \left(|\Delta(x)| + \CK L h(x)^\alpha \right)^2 dx \right]^2 \nonumber \\
    & \leq 8\left[\int_\B \omega(x)|\Delta(x)|^2 dx \right]^2 + 8\left[\int_\B \omega(x)\CK^2 L^2 h(x)^{2\alpha} dx \right]^2 \nonumber\\
    & = 8J^2 + 8 \CK^4 t_n^2.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ancienne expression de la variance dans le lemme (pas suffisant)
\begin{align*}
    \V(\Tb) \leq& \; 16\, \CK^4 t_n^2 + 16 J^2 + \frac{2}{k^2}\iint_{\B^2} \omega(x) \omega(y) \text{cov}^2\left(K_{h(x)}(x-X),K_{h(y)}(y-X)\right)  dx dy.
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ancienne preuve que $\E \Tb \gtrsim J$
 We have $ \E[\Tb] = \int_\B \omega(x) \E\left[ \hat \Delta (x)\right]^2dx$. Moreover,
\begin{align}
    \E\left[\hat \Delta (x)\right]^2 &= \left[p(x)-p_0(x)+\E\left(\hat p(x) - p(x)\right)\right]^2 \nonumber \\
    &\geq \frac{1}{2} \left[p(x)-p_0(x)\right]^2 - \left[\E\left(\hat p(x) - p(x)\right)\right]^2 \label{exp_Delta_squared}
\end{align}

by the inequality $(a+b)^2 \geq a^2/2 - b^2$.
First,
\begin{align*}
    \left[\E\left(\hat p(x) - p(x)\right)\right]^2 \leq L^2\hB(x)^{2\alpha}
\end{align*}
so by Lemma \ref{omega_h_2alpha}, 
\begin{equation}\label{biais_expectation_H1}
    \int_\B \omega(x) \left[\E\left(\hat p(x) - p(x)\right)\right]^2dx \leq t_n.
\end{equation}


with 
\begin{align}
    \int_\B \frac{1}{\omega^\frac{t}{2-t}}\;\;\; &=\;\;\; \int_\B p_0^\frac{2\alpha t}{(4-t)\alpha + d}\left(L^2 \I \right)^\frac{dt}{(2-t)(4\alpha + d)}\nonumber \\
    \text{i.e. } \;\;\; \left(\int_\B \frac{1}{\omega^\frac{t}{2-t}}\right)^{-\frac{2-t}{t}} &= \;\;\;L^{-\frac{2d}{4\alpha + d}} \I^{-\frac{8\alpha + 2d - 4\alpha t}{t(4\alpha + d)}}\label{1_over_int}
\end{align}


By \eqref{1_over_int}, \ref{biais_expectation_H1} and \eqref{L2_estim_t_norm}, we get $J \geq (\RadB^2-1) t_n$. Therefore, by equation \eqref{exp_Delta_squared}:
\begin{align*}
    \mathbb{E}[\Tb] \geq \big(\frac{1}{2} - \frac{1}{\RadB - 1} \big)J \geq \frac{1}{4} J
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


First, by triangular inequality,
\begin{align*}
    \left|\E\left[K_{h(x)}(x-X) - p_0(x)\right]\right| \; \leq \; |p(x)-p_0(x)| + \big|\E\left(\hat p(x) - p(x)\right)\big| \; \leq \; |\Delta(x)| + \CK L h(x)^\alpha
\end{align*}

\ju{
When we plug into \eqref{var_bulk_H1} we get:
\begin{align}
    \V(\Tb) & \leq \iint_{\B^2} \omega(x) \omega(y) \E\left[\hat \Delta(x) \hat \Delta(y)\right]^2 dx dy\\
    & \leq \iint_{\B^2} \omega(x) \omega(y) \left[2  \right] dx dy
\end{align}
$\left[\left(p(x)-p_0(x)\right)\left(p(y)-p_0(y)\right)\right]^2$ into the integral, we directly get $\V \leq \E^2$. Idem when plugging $\left[L^2 h(x)^\alpha h(y)^\alpha\right]^2$. Cross terms: no problem.\\
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ancienne analyse de la covariance sous H0 bulk
\begin{align*}
      & + 3 \iint_{\B^2} \omega(x)\omega(y) \left[ \mathbb{1}_{\D^c} \frac{1}{k} \Big(\frac{\CK}{\cA} +1 \Big)^2 p_0(x) p_0(y) \right]^2 dxdy ~~ \text{ (Term II)}\\
  & + 3 \iint_{\B^2} \omega(x)\omega(y) \left[\mathbb{1}_\D \Cclose \frac{p_0(x)}{k \; h(x)^d } \right]^2 dxdy ~~~~~~~~~~~~~~~~~~~~~ \text{ (Term III)}
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Concentration du prior tail en $\rhot$ autour de $p_0$.

\begin{proof}[Proof of Proposition \ref{separation_prior_tail}]
Assume throughout the proof that $\int_{\B^c} p_0 > \frac{\ctail}{n}$. We show that our prior concentrates with high probability on a zone separated away from $p_0$ by an $L^t$ distance of order $\rhot$, up to an absolute constant. To do so, we compute the expectation and the variance of $\|p_0 - p_b\|_t^t$. We then apply Chebyshev's inequality to show that this quantity concentrates on the desired zone. We will use the notation $Z = \|p_0 - p_b\|_t^t$, $S = \int_{\B^c}p_0$ and $\gamma = \|\gamma_1\|_t = \dots = \|\gamma_M\|_t$ \ju{Attention imprécision dans la définition de $\gamma$, c'est plutôt le prior mis sur toute la case !}.
\begin{align*}
    \mathbb{E}[Z] &= \mathbb{E}\big[ \sum_{j=1}^M b_j^t\gamma^t\big] = \gamma^t \sum_{j=1}^M \lambda ~~ = ~~ \gamma^t n^2S^2.\\
    \mathbb{V}[Z] &= \mathbb{V}\big[ \sum_{j=1}^M b_j^t\gamma^t\big] = \gamma^{2t} \sum_{j=1}^M \lambda(1-\lambda) \leq  \gamma^{2t} n^2S^2.
\end{align*}

\ju{Quand on met aussi la compensation avec le bulk ça fait sortir un facteur $2$ en plus.}

Therefore, by Chebyshev's inequality, with probability at least $1-\eta/4$:
\begin{align*}
    &|Z - \mathbb E[Z]| \leq \frac{2}{\sqrt{\eta}}\sigma(Z) ~~ \Longrightarrow ~~ Z \geq \mathbb E[Z] - \frac{2}{\sqrt{\eta}}\sigma(Z)  ~~ \text{ where } \sigma(Z) = \sqrt{\mathbb{V}(Z)} \\
    & \Longrightarrow ~~ Z \geq \gamma^t n^2 S^2 - \frac{2}{\sqrt{\eta}}\gamma^t n S \geq \gamma^t \, \frac{n^2 S^2}{2} ~~ \text{ since for } S \geq \ctail : n^2S^2 - \frac{2}{\sqrt{\eta}} nS \geq \frac{n^2 S^2}{2}
\end{align*}

Now
\begin{align*}
    \gamma^t = \int_{[-\frac{h}{2}, \frac{h}{2}]} {\cgamma}^t L^t \big(h - \|x\| \big)_+^{\alpha t} dx = {\cgamma}^t L^t h^{\alpha t +d} \int_{\R^d} (1- \|y\|)_+^{\alpha t} dy =: \Ctgamma L^t h^{\alpha t + d}.
\end{align*} so that
$$ \frac{1}{2}\gamma^t n^2 S^2 = \frac{1}{2}\Cgamma \rhot(\uI).$$
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Disjonction de cas pour prouver que mettre le prior tail sur tuote la case c'est pareil que d'intersecter avec le tail.

$C_U \subsetneq \widetilde C_U$. Then necessarily, there exists $j \in \widetilde C_U$ such that $p_0(z) > \uA$. By assumption \eqref{simplifyingAssumption}, we have:
    \begin{align*}
        p_U &\geq \int_{\widetilde C_U} p_0(z) - \cstar L\|z - x\|^\alpha dx = p_0(z) h^d - \cstar L h^{\alpha + d}\\
        &  \geq L (\cA  \hB(z)^\alpha - \cstar h^\alpha)h^d \geq L(\cA - \cstar)h^{\alpha + d} ~~ \text{ by Lemma \ref{htail_leq_hbulk}}  \\
        &= (\cA - \cstar) \frac{1}{n^2 \int_{\T(\uA)} p_0}.
    \end{align*} 
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Remarque cases tail

Attention, on met le prior sur toute la case, même si un bout de la case est dans le bulk. Dans ce cas ça veut dire que pour la borne sup on doit plutôt définir une autre tail qui correspond à tous les cubes (non intersectés avec le tail) et montrer qu'elle ne change pas le rate. On a donc besoin d'un lemme qui dit ça. 

\ju{de plus il y a un autre problème : on dit que le tail est $\{p_0 < \uI\}$ puis on le découpe en petits cubes. Cela revient à d'abord découper en cubes puis à intersecter avec $\{p_0 < \uI\}$. Ca veut dire qu'il peut y avoir des cases à cheval sur bulk et tail. Cependant, là on met le prior sur \textbf{toute la case} sans se soucier du fait qu'elle soit totalement incluse dans le tail. Il faut donc prouver que les cas éventuellement problématiques ne le sont en fait pas.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preuve que $\lambda \leq 1$

\begin{proof}[Proof of Lemma \ref{lambda_leq_1}]
Set $h = \hT(\uA)$. By the Cauchy-Schwarz inequality:
$$ \frac{1}{|\B^c|} \Big(\int_{\B^c} p_0 \Big)^2 \leq \int_{\mathcal T(\uI)} p_0^2 \leq \frac{\Cmom}{n^2h^d} \text{ by definition of $\uI$}$$
Therefore:
$$ \lambda = \frac{1}{M}\Big( n  \int_{\B^c} p_0\Big)^2 \leq \frac{1}{M} \frac{\Cmom |\B^c|}{h^d} \leq \frac{1}{M} \Cmom M\leq 1$$ .
\end{proof}

\hfill

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% idée de la diagonale avec une fenêtre plus petite pour le noyau

 Pour ce terme peut-être qu'il faut prendre une autre constante dans la def de la diagonale : ça permet de virer plein de masse en dehors de la diagonale. Puis sur la diagonale, c'est la même chose avec une autre constante. Ca revient à prendre une Kernel avec une fenêtre une constante multiplicative plus grande.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%
 \ju{expliciter $\cstar$, on a besoin de $\frac{\cstar}{\cA} \ll 1 $ cf Lemme \ref{const_balls}, ça devrait autoriser $\cstar$ à être $\gg 1$ ?}
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
\begin{align*}
    & \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) \text{cov}^2\left(K_{h(x)}(x-X),K_{h(y)}(y-X)\right)  dx dy \\
     \leq & \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) \Big[\Ccov p_0(x) + |\Delta(x)| \Big]^2 \Big[\Ccov p_0(y) + |\Delta(y)| \Big]^2 dx dy\\
     = & \frac{1}{k^2}\int_{\B} \omega(x) \Big[\Ccov p_0(x) + |\Delta(x)| \Big]^2 \Big\{\underbrace{\int_{\mathcal{D}(x)^c} \omega(y) \Big[\Ccov p_0(y) + |\Delta(y)| \Big]^2 dy}_{:=J(x)}\Big\} dx\\
\end{align*}

\ju{Changer tous les $D(x)$ en $D(x)^c$}

Now, for fixed $x \in \B$, by Minkowski's inequality:
\begin{align*}
    J(x)& \leq \Big[\Ccov\sqrt{\int_{D(x)} \omega(y) p_0^2(y) dy} + \sqrt{\int_{D(x)} \omega(y) \Delta^2(y) dy } \; \Big]^2\\
    & \leq \Big[\Ccov\sqrt{t_n} + \sqrt{\int_{D(x)} \omega(y) \Delta^2(y) dy } \; \Big]^2 ~~ \text{ by Lemma \ref{omega_h_2alpha}}.
\end{align*}

Therefore,
\begin{align*}
    J_{\D^c} &\leq \frac{1}{k^2}\int_{\B} \omega(x) \Big[\Ccov p_0(x) + |\Delta(x)| \Big]^2  \Big[\Ccov\sqrt{t_n} + \sqrt{\int_{D(x)} \omega(y) \Delta^2(y) dy } \; \Big]^2 dx\\
    & \leq \frac{1}{k^2} \Bigg(\sqrt{\int_{\B} \omega(x) \big(\sqrt{t_n} + \sqrt{J} \big)^2 p_0^2} + \dots \Bigg)^2
\end{align*}

\ju{On peut terminer mais sans doute que ça sert à rien, le calcul d'en dessous est plus simple}

\hfill \break  \break \break

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{align*}
    & \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) L^2 h^{2\alpha}(x)p^2(y) dx dy \leq \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) L^2 h^{2\alpha}(x)\left[2 p_0^2(y) + 2|\Delta(y)|^2 \right] dx dy\\
    & \leq \frac{2}{k^2\cA^2} \iint_{\D^c} \omega(x)\omega(y) \, p_0^2(x) p_0^2(y) \, dx dy + \frac{2}{k^2}\int_{\B} \omega(x) L^2h^{2\alpha}(x) dx \int_\B \omega(y)|\Delta(y)|^2 dy\\
    & \leq \frac{8}{\cA^2\cp } t_n^2 + \frac{2}{k^2} t_n J ~~ \text{ by Lemmas \ref{control_xy_far} and \ref{omega_h_2alpha}},
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preuve fausse que $\int(p-p_0)^2 \lesssim \sum q_j^2/h^d$

\ju{Reprendre complètement ! LEs équations \eqref{abs_p-p0_x} et \eqref{abs_p-p0_x_j} ont l'air fausses et de plus j'ai changé \eqref{simplifyingAssumption} en mettant le $\cstar$ seulement sur le $p$.}

By the triangular inequality, $|p-p_0|$ satisfies Assumption \eqref{simplifyingAssumption} with the constants $2L$ and $2\cstar$, so that for all $j=1, \dots, M$ and for all $x \in \mathcal{T}$, upper-bounding the maximum by the sum yields:
\begin{equation}\label{abs_p-p0_x}
    |p-p_0|(x) \leq (2\cstar+1)|p-p_0|(x_j) + 2 L \; \|x - x_j\|^\alpha
\end{equation}
and 
\begin{equation}\label{abs_p-p0_x_j}
    |p-p_0|(x_j) \leq (2\cstar+1)|p-p_0|(x) + 2L \; \|x - x_j\|^\alpha
\end{equation}
Fix $j \in \{1, \dots, M\}$. Writing $h$ for $\hT(\uA)$ we have:
\begin{align*}
    \int_{C_j} (p-p_0)^2 &\leq 2\, \cstar\left(\int_{C_j}\abs{p-p_0}\right) \abs{p - p_0}(x_i) + 2 L \; h^\alpha\int_{C_j}\abs{p-p_0} ~~ \text{ by \eqref{abs_p-p0_x}} \\
    & \leq \left(\int_{C_j}\abs{p-p_0}\right) \left[\frac{1}{h^d}\int_{C_j}\abs{p-p_0} + 2\, \cstar Lh^\alpha\right] + 2\, \cstar Lh^\alpha\int_{C_j}\abs{p-p_0} \\
    & = \frac{1}{h^d}\left(\int_{C_j}\abs{p-p_0}\right)^2 + 4 \cstar Lh^\alpha\int_{C_j}\abs{p-p_0} \\ & \leq \frac{2}{h^d}\left(\int_{C_j}p\right)^2 + \frac{2}{h^d}\left(\int_{C_j}p_0\right)^2 + 4 \cstar Lh^\alpha\int_{C_j}\abs{p-p_0} \\
    & \leq \frac{2}{h^d}\left(\int_{C_j}p\right)^2 + 2 \int_{C_j} p_0^2 + 4 \cstar Lh^\alpha\int_{C_j}\abs{p-p_0}
\end{align*}

The result is obtained by summing over $j=1,\dots, M$ and recalling that, by lemma \ref{int_p0squared_uA_small}, $\int_{\B(\uA)^c} p_0^2 \leq \Cmom \frac{1}{n^2\barhT^d} \leq \Cmom \frac{1}{n^2\hT^d(\uA)}$, no matter whether $\uA = \uI$ or $\uA > \uI$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our goal is now to set a sparse prior. The first step is to remove from \textit{each cube} $\widetilde C_j$, $j\geq U$ some constant fraction of the mass $\int_{\widetilde C_j}p_0$. To do so, we place ourselves on each $\widetilde C_j$ and subtract from $p_0$ a suitable deterministic function $\gammadown_j \in H(\alpha, \delta' L)$, where $\delta'$ \ju{Compléter}. The second step consists in selecting a sparse random subset $J_S \subset \{U,\dots,M\}$ and in adding to each cube $\widetilde C_j, \,j \in J_S$, one large perturbation. To do so, we draw independently for any cube $\widetilde C_j, \, j \geq U$ one Bernoulli random variable $b_j \sim Ber(\pi_j)$ and add the large perturbation $\gammaup_j \in H(\alpha, \delta' L)$ whenever $b_j=1$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition}\label{prior_tail_admissible}
For all $b \in \{0,1\}^M$: $p_b \in \mathcal{P}(\alpha, L)$. \ju{attention, plutôt $(1+\delta) L$}. \ju{Vérifier \eqref{simplifyingAssumption}.}
\end{proposition}

\hfill

\begin{proof}[Proof of Proposition \ref{prior_tail_admissible}]
For all $j \geq U: \gamma_j \in H(\alpha, \cgamma L)$ and all $(\gamma_j)_j$ have disjoint supports. It follows that $p_b \in H(\alpha, L(1+\cgamma))$ for all $b \in \{0,1\}^M$ \ju{faire le lien avec $\delta$}. Moreover, $p_b \geq 0$ is clear. \ju{Il manque la compensation sur le bulk pour $\int = 1$}. \ju{Attention j'ai peut-être changé la définition de $\cgamma$.}
\end{proof} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lemma Poisson normalisé et dénormalisé.

\begin{lemma}\label{TVpoisson_TVdenorm}
\ju{Modifier} Let $\lambda \in (0,1)$ and $\AnormQ = \big\{\|q_b\|_1 \in \big[\frac{1}{1 \mp \lambda} \big]\big\}$. It holds $d_{TV}(\bar p^{(\widetilde n)}, p_0^{\otimes \widetilde n}) \leq d_{TV}(q^{(\widetilde n)}, p_0^{\otimes \widetilde n}) + \lambda + \mathbb{P}(\AnormQ^c)$. \ju{Attention il y a sûrement un raffinement à apporter avec le bulk. De plus, choisir $\lambda$ de sorte que le terme résiduel soit petit.}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{TVpoisson_TVdenorm}]
Let $\lambda \in (0,1)$ and $\AnormQ = \big\{\|q_b\|_1 \in \big[\frac{1}{1 \mp \lambda} \big]\big\}$. We have:
\begin{align*}
    d_{TV}(\bar p^{(\widetilde n)}, p_0^{\otimes \widetilde n}) \leq \sup_{A \in \Xtilde \cap \AnormQ} \big|\bar p^{(\widetilde n)}(A) - p_0^{\otimes \widetilde n}(A) \big| + \mathbb{P}(\AnormQ^c).
\end{align*}
Let $A_0 \in  \Xtilde \cap \AnormQ$ such that $\big|\bar p^{(\widetilde n)}(A_0) - p_0^{\otimes \widetilde n}(A_0) \big| = \sup_{A \in \Xtilde \cap \AnormQ} \big|\bar p^{(\widetilde n)}(A) - p_0^{\otimes \widetilde n}(A) \big|$. \ju{Est-ce qu'on a le droit de le fixer ? Sinon on fait un truc avec des $\epsilon$.} There are two cases:
\begin{enumerate}
    \item If $\bar p^{(\widetilde n)}(A_0) \geq p_0^{\otimes \widetilde n}(A_0)$ then
    \begin{align*}
        \big|\bar p^{(\widetilde n)}(A_0) - p_0^{\otimes \widetilde n}(A_0) \big| &= \bar p^{(\widetilde n)}(A_0) - p_0^{\otimes \widetilde n}(A_0) \leq (1+\lambda)q_b^{(\widetilde n)}(A_0) - p_0^{\otimes \widetilde n}(A_0) \\
        &\leq d_{TV}\big(q_b^{(\widetilde n)}(A_0), \; p_0^{\otimes \widetilde n}(A_0) \big) + \lambda.
    \end{align*}
    \item Otherwise:
    \begin{align*}
        \big|\bar p^{(\widetilde n)}(A_0) - p_0^{\otimes \widetilde n}(A_0) \big| &= p_0^{\otimes \widetilde n}(A_0) - \bar p^{(\widetilde n)}(A_0) \leq p_0^{\otimes \widetilde n}(A_0) -  (1-\lambda)q_b^{(\widetilde n)}(A_0) \\
        &\leq d_{TV}\big(q_b^{(\widetilde n)}(A_0), \, p_0^{\otimes \widetilde n}(A_0) \big) + \lambda.
    \end{align*}
\end{enumerate}
In both cases, the result is proven.
\end{proof}

\vspace{3cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{3cm}


We define the subset $\A \subset \Omega^n$ as the set of observations $(x_1,\dots,x_n)$ such that any cell $C_j, j=1, \dots, M$ contains at most one observation:
\begin{equation}\label{def_A}
    \A := \{(x_1, \dots, x_n) \in \Omega^n: \forall j=1,\dots, M, N_j \leq 1\}
\end{equation} where $N_j$ is defined in \eqref{Nj}. By Lemma \ref{proba_observed_twice}, this set has probability at least $1-\Cmom$. By Lemma \ju{Donner le Lemme}, this set has probability at least $1 - \Cpbar$ under the prior (where $\Cpbar$ is given in Lemma \ju{Compléter}). \ju{On a besoin d'un Lemme qui calcule la proba de $\A$ sous le prior.} We therefore have:
\begin{align*}
    d_{TV}(\mathbb{P}_{p_0}, \mathbb{P}_{\bar p}) &= \frac{1}{2}\int_{\Omega^n} \left|p_0^{\otimes n}(x_1, \dots, x_n) - \bar p(x_1, \dots, x_n)\right|dx_1\dots dx_n\\
    &\\
    & \leq \frac{1}{2}\int_{\mathcal{\A}} \left|p_0^{\otimes n}(x_1, \dots, x_n) - \bar p(x_1, \dots, x_n)\right|dx_1\dots dx_n \,+\, \frac{1}{2}\mathbb{P}_{p_0}(\A^c) \,+ \, \frac{1}{2}\mathbb{P}_{\bar p}(\A^c)\\
    &\\
    & \leq \frac{1}{2}\int_{\mathcal{\A}} \left|p_0^{\otimes n}(x_1, \dots, x_n) - \bar p(x_1, \dots, x_n)\right|dx_1\dots dx_n + \frac{1}{2}\Cmom + \frac{1}{2}\Cpbar.
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preuve Lemme \ref{TV_over_A}
Moreover, by the triangular inequality:
\begin{align*}
    \sup_{A \in \widetilde X \cap \Aonce} \big| \qtens(A) - \ptens(A)\big| \leq& \left[\sup_{A \in \widetilde X \cap \Aonce} \big| \qtens(A| \Aonce) - \ptens(A | \Aonce)\big| \right] \ptens(\Aonce) \\
    &+ \left[\sup_{A \in \widetilde X \cap \Aonce}  \qtens(A| \Aonce) \right]\big| \qtens(\Aonce) - \ptens(\Aonce) \big|\\
    & \leq d_{TV}(\qtens\left(\cdot | \Aonce\right), \ptens(\cdot | \Aonce)) + \qtens(\Aonce^c)+ \ptens(\Aonce^c).
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preuve Lemme \ref{Tensorization _Poisson}
\hfill

$\Poi(2np_{0,\Aonce})= \bigotimes_{j=1}^{M+1} \Poi(2np_{0 | \widetilde C_j, \Aoncej})$ and $\Poi(2nq_{b, \Aonce}) = \bigotimes_{j=1}^{M+1} \Poi(2nq_{b_j| \widetilde C_j, \Aoncej})$. \ju{Attention avec $M+1$} Hence our last quantity can be upper bounded as $d_{TV}\big(\Poi(2nq_{b_j| \widetilde C_j}(\cdot | \Aonce)), \ptens(\cdot | \Aonce)\big) \leq \sum_{j=1}^{M+1} d_{TV}\big(\Poi(2n q_{b| \widetilde C_j}(\cdot | \Aoncej)), \Poi(2np_{0 | \widetilde C_j})(\cdot | \Aoncej))\big)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{3cm}

To do so, we compute the expectation and the variance of $\|p_0 - p_b\|_t^t$. We then apply Chebyshev's inequality to show that this quantity concentrates on the desired zone. We will use the notation $Z = \|p_0 - p_b\|_t^t$, $S = \int_{\B^c}p_0$ and $\gamma = \|\gamma_1\|_t = \dots = \|\gamma_M\|_t$ \ju{Attention imprécision dans la définition de $\gamma$, c'est plutôt le prior mis sur toute la case !}. \\

By Lemma \ref{I_and_U}, we are necessarily in the case $\int_{D(U)} p_0 \geq \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0$. Indeed, if $\int_{D(U)} p_0 < \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0$, we would have by Lemma \ref{I_and_U}:
\begin{align*}
    \int_{\mathcal{T}(\uI)} p_0 &\leq \int_{D(U)} p_0 + \frac{\sqrt{\cI}}{n}\\
    & < \frac{1}{3} \int_{\mathcal{T}(\uI)} p_0 + \frac{\sqrt{\cI}}{n}
\end{align*} hence: $\int_{\mathcal{T}(\uI)} p_0 \leq \frac{3}{2}  \frac{\sqrt{\cI}}{n}$ which is excluded since we assume $\int_{\mathcal{T}(\uI)} p_0 \geq \frac{\ctail}{n}$.\\

\ju{finir}


%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{I_and_U} \ju{Enlever} It holds : $$\int_{D(U)} p_0 + \frac{1}{n} \asymp \int_{\mathcal{T}(\uI)} p_0 + \frac{1}{n}.$$ Moreover, we either have $$\int_{D(U)} p_0 \geq \frac{1}{3}\int_{\mathcal{T}(\uI)} p_0 ~~ \text{ or } ~~ \int_{\mathcal{T}(\uI)} p_0 \leq \int_{D(U)} p_0 + \frac{\sqrt{\cI}}{n}$$
\end{lemma}

\begin{proof}[Proof of Lemma \ref{I_and_U}]
\ju{Enlever}
\ju{Problème avec l'intersection cases/tail}
In this proof, we will use the following notation:
$$\forall j =1, \dots, M: ~p_j:= \int_{C_j} p_0.$$
\vspace{-8mm}
\begin{align*}
     S ~~ &:=~ \sum_{j=1}^M p_j = \int_{T(\uI)} p_0 \\
     S_U ~ &:=~ \sum_{j \geq U} p_j = \int_{D(U)} p_0 \\
    S_{-U} &:=~ S - S_U\\
    h ~ & ~ = \hT(\uI)
\end{align*}
We want to prove $S + \frac{1}{n} \asymp S_U + \frac{1}{n}$ and $\big[ S_U \geq \frac{1}{3} S \text{ or } S \leq S_U + 2\frac{\sqrt{\cI}}{n} \big]$.
If $S_U \geq S/3$ then the result is clear. Assume $S_U < S/3$. Then $S_U < \frac{1}{2} S_{-U}$. Let $V \in \{1, \dots, U-1\}$, then:
\begin{align*}
    \int_{C_V} p_0^2 + \frac{1}{2} \frac{\cI}{n^2 h^d} &\geq \int_{C_V} p_0^2 + \frac{1}{2}\int_{\mathcal{T}(\uI) \setminus D(U)} p_0^2 ~~ \text{ by definition of } \uI\\
    &\\
    & \geq \frac{1}{h^d}\, p_V^2 + \frac{1}{2} \sum_{j < U} \frac{1}{h^d} \, p_j^2 ~~ \text{ by the Cauchy-Schwarz inequality}\\
    & > \frac{p_{U-1}}{h^d} \big(p_{U-1} + \sum_{j \geq U} p_j\big) ~~ \text{ since } S_U < \frac{1}{2} S_{-U}\\
    & > \frac{\cu}{n^2h^d} ~~ \text{ by definition of }U.
\end{align*}
Therefore, it holds for all $V < U$:
\begin{equation}\label{CV}
    \int_{C_V} p_0^2 > \frac{\cu - \cI/2}{n^2 h^d} \geq \frac{\cI}{2n^2 h^d}
\end{equation}
Moreover by definition of $\uI$:
\begin{align*}
    \frac{\cI}{n^2h^d} \geq \int_{\mathcal{T}(\uI) \setminus D(U)} p_0^2 = \sum_{j<U} \int_{C_j} p_0^2 > (U-1)\frac{\cI}{2n^2h^d} ~~\text{ by  \eqref{CV}}
\end{align*}
Therefore: $U \leq 2$ so $U=2$ since otherwise we would not have $S_U < S/3$. Then
\begin{align*}
    S = p_1 + S_U \leq \sqrt{h^d \int_{C_1}p_0^2} + S_U \leq \frac{\sqrt{\cI}}{n} + S_U
\end{align*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{align*}
    & \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) \text{cov}^2\left(K_{h(x)}(x-X),K_{h(y)}(y-X)\right)  dx dy \\
    & \leq \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) \left[\CK^2 L^2 h^\alpha(x) h^\alpha(y) + 2 \CK Lh^\alpha(x) p(y) + p(x)p(y) \right]^2 dx dy \\
    & \leq \frac{3 \CK^4}{k^2} \left[\int_{\B} \omega(x) L h(x)^{2\alpha} dx \right]^2 + \frac{3 }{k^2}\iint_{\D^c} \omega(x) \omega(y) \left[4\CK^2L^2 h^{2\alpha}(x)p^2(y) + 2p^2(x) p^2(y) \right] dx dy\\
    & \leq \frac{3 \CK^4}{k^2} t_n^2 + \underbrace{\frac{12 \CK^2}{k^2}\iint_{\D^c} \omega(x) \omega(y) L^2 h^{2\alpha}(x)p^2(y) dx dy}_{\text{Term IV}} + \underbrace{\frac{6}{k^2} \iint_{\D^c} \omega(x) \omega(y) p^2(x) p^2(y) dx dy}_{\text{Term V}}.
\end{align*}
At the third inequality we have used $(a+b+c)^2 \leq 3(a^2+b^2+c^2)$ and at the fourth, Lemma \ref{omega_h_2alpha}.\\

\underline{\textbf{Term IV:}} 
\begin{align*}
     & \frac{1}{k^2}\iint_{\D^c} \omega(x) \omega(y) L^2 h^{2\alpha}(x)p^2(y) dx dy \leq \frac{4}{n^2}\left[ \int_{\B} \omega L^2 h^{2\alpha} \int_\B \omega p^2 \right]\\
     \leq & \frac{4}{n} t_n \left[\frac{2}{\sqrt{\cp}}t_n + \frac{2}{n}J \right] = \frac{8}{n \sqrt{\cp}}t_n^2 + \frac{8}{n^2} t_n J  ~~ \text{ by Lemmas \ref{control_xy_far} and \ref{omega_h_2alpha}},
\end{align*}


so that:
\begin{align*}
    \frac{12 \CK^2}{k^2}\iint_{\D^c} \omega(x) \omega(y) L^2 h^{2\alpha}(x)p^2(y) dx dy \leq \frac{96\CK^2}{n \sqrt{\cp}}t_n^2 + \frac{96\CK^2}{n^2} t_n J.
\end{align*}

\hfill \break

\underline{\textbf{Term V}} : 
\begin{align*}
    &\frac{6}{k^2} \iint_{\D^c} \omega(x) \omega(y) p^2(x) p^2(y) dx dy \leq 24 \left(\frac{1}{n}\int_\B \omega p^2 \right)^2 \leq 24 \left(\frac{2}{\sqrt{\cp}} t_n + \frac{2}{n}J \right)^2 \text{ by Lemma \ref{int_omega_p2}}\\
    &\leq 200 \left(\frac{t_n^2}{\cp} + \frac{J^2}{n^2} \right).
\end{align*}

\begin{align*}
    \leq 200 \left(\frac{t_n^2}{\cp} + \frac{J^2}{n^2} \right).
\end{align*}

Therefore:
\begin{equation}\label{Majorant_JDc}
    J_{\D^c} \leq \left(\frac{12\CK^4}{n^2} + \frac{96 \CK^2}{n\sqrt{\cp}} + \frac{200}{\cp}\right) t_n^2 + \frac{96 \CK^2}{n^2} t_n J + \frac{200}{n^2}J^2.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Explication algorithme dans le cas du bulk

For the lower bound on bulk, we will need to partition $\B$ into cubes of optimal edge lengths, using an algorithm similar to \cite{balakrishnan2019hypothesis}, Algorithm 1. Assume that $\B \neq \emptyset$. The partitioning algorithm splits the bulk recursively: At step $0$, we define one single cube $B^{(0)} = [0,1]^d$. Then each cube $B^{(j)}$ is split into $2^d$ smaller cubes obtained by halving the original $B^{(j)}$ along each of its axes, and any new cube with empty intersection with $\B$ is removed. We repeat until the following condition is satisfied: $\text{diam } B^{(j)} \leq \cSplitBulk \cdot \hB(x)$ where $x \in \arg\max_{B^{(j)}} p_0$. \ju{Est-ce que c'est le max ou la valeur au centre ? Donner $c$. Attention c'est pas vraiment le diamètre c'est plutôt le côté.} If this condition is met, nothing is done to $B^{(j)}$. When all the cubes satisfy this condition, order the family of cubes thus defined as $(B_1, \dots, B_N)$ for some $N \in \N$. %, and define for all $j=1, \dots, N: B_j = A_j \cap \B$. \ju{Donner la valeur de $\cSplitBulk$. Est-ce qu'on donne l'algorithme de partition plus précisément ? Justifier que l'algo termine et que les cubes sont bien tq si centré à $x$ alors de diamètre $\asymp c h(x)$.}\\
For any $j$, we denote by $x_j$ the center of $B_j$. Each cube $B_j$ therefore has edge length $\leq c\hB(x_j)$, is centered at $x_j$ and satisfies $B_j \cap \B \neq \emptyset$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% split plus findes cases tail

\ju{Définir un algorithme qui prend en entrée un cube, une partie $\mathcal{D}$ du cube et une fonction $p_0 \geq 0$ définie dessus, une fonction $h \geq 0$ définie dessus et fait un partitionnement hiérarchique en cubes centrés en $x_i$ de côté $h(x_i)$. Ca veut dire qu'on peut l'appliquer dans la BI du bulk avec $[0,1]^d$, $\B$, $p_0$ et $\hB$ et dans la BI tail avec $\widetilde C_j$, $D_j$, $p_0$ et $h(x) = (p_0/L)^\frac{1}{\alpha}$.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Split plus fin des cases tail

\ju{Définir un algorithme qui prend en entrée un cube, une partie $\mathcal{D}$ du cube et une fonction $p_0 \geq 0$ définie dessus, une fonction $h \geq 0$ définie dessus et fait un partitionnement hiérarchique en cubes centrés en $x_i$ de côté $h(x_i)$. Ca veut dire qu'on peut l'appliquer dans la BI du bulk avec $[0,1]^d$, $\B$, $p_0$ et $\hB$ et dans la BI tail avec $\widetilde C_j$, $D_j$, $p_0$ et $h(x) = (p_0/L)^\frac{1}{\alpha}$.}

%%%%%%%%%%%%%%%%%%%%
 is defined using a partitioning scheme, adapted from that used in the bulk lower bound. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{proba_twice_H1_tail}
Let $h = \hT(\uA)$. Under the prior \eqref{def_prior_tail}, the probability that at least one of the cells $(C_j)_{j=1,\dots,M}$ contains at least two observations is upper bounded as
\begin{align*}
    \mathbb{P}_{p_b^{(n)}}[\, \exists j \in \{1, \dots, M\}: N_j \geq 2\, ] \leq 2 \Cmom + {\Cgamma}^2.
\end{align*}
\end{lemma}


\begin{proof}[Proof of Lemma \ref{proba_twice_H1_tail}]
We place ourselves under the prior \eqref{def_prior_tail}. For all $j = 1, \dots, M$, let $q_j = \int_{C_j} p_0$ and let $\gamma = \int_{C_j} \gamma_j =: \Cgamma L h^{\alpha + d}$ where $\Cgamma = \cgamma\int_{\R^d} (1 - \|y\|)^\alpha dy$. Fix $b \in \{\pm 1\}^M$ and define $q_j(b) = q_j + b_j \gamma$. By the definition of $N_j = \sum_{i=1}^n \mathbb{1}\{X_i \in C_j\}$, we have $N_j \sim Bin(q_j(b),n)$ for all $j=1, \dots, M$. Therefore the probability that for a fixed $j$, $N_j$ is at least $2$ is upper bounded as:
\begin{align*}
    1 - (1-q_j(b))^n - nq_j(b)(1-q_j(b))^{n-1} \leq 1 - (1-nq_j(b)) - nq_j(b)[1-(n-1)q_j(b)] \leq n^2q_j(b)^2
\end{align*}
The probability that at least one of the $N_j$ is at least $2$ is therefore upper bounded as $\sum_{j=1}^M n^2q_j(b)^2$.

Therefore:
\begin{align*}
    &\mathbb{P}_{p_b^{(n)}}[\, \exists j \in \{1, \dots, M\}: N_j \geq 2\, ] \leq \mathbb{E}_{b_j \overset{iid}{\sim} Ber(\lambda))}\big[ n^2q_j(b)^2\big]\\
    & \leq n^2 \sum_{j=1}^M \lambda \large(q_j + \gamma \large)^2 + 2(1-\lambda) q_j^2 \leq n^2 \sum_{j=1}^M \Large(2q_j^2 + \lambda \gamma \Large) \leq  2 \Cmom + {\Cgamma}^2,
\end{align*}
by Lemma \ref{proba_observed_twice} and the definition of $\lambda$, $\gamma$ and $h$.

\ju{Vérifier subtilité entre $\hT(\uI)$ et $\hT(\uA)$.}

\end{proof}
%%%%%%%%%%%%%%%%%%%%%%

    
    
    Since $p_0$ is continuous, let $z_j \in \widetilde C_j$ such that $p_0(z_j) h^d = p_j$. Then necessarily, $p_0(z_j) \leq \Cstep Lh^\alpha$. We therefore have:
    \begin{align*}
        p_j \leq \int_{\widetilde C_j} p_0(z_j) + \Cstep L h^{\alpha} dx \leq 2\Cstep L h^{\alpha + d} < p_U.
    \end{align*}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Set $h = \hT(\uA)$, $v :=  \frac{2}{\cA}\uA$ and let $J_{\text{large}} = \{j \geq U:  \text{ s.t. } \sup_{\widetilde C_j} p_0 \geq v\}$.
\begin{itemize}
    \item For all $j \in \{1,\dots,M\} \setminus J_{\text{large}}$, we have: $\sup_{\widetilde C_j} p_0 < v \leq \uA$, hence $\bigcup_{j \notin J_{\text{large}}} \widetilde C_j \subset \T(\uA)$, which yields by Lemma \ref{int_p0squared_uA_small}: $\int_{\bigcup_{j \notin J_{\text{large}}} \widetilde C_j} p_0^2 \leq \frac{\Cmom}{n^2 h^d}$.
    \item For all $j \in J_{\text{large}}$,let $y_j \in \widetilde C_j$ such that $p_0(y_j) > v$. By Assumption \ref{simplifyingAssumption} we have for all $x \in \widetilde C_j: p_0(x) \geq p_0(y_j) - L h^\alpha \lor \cstar p_0(y_j) \geq p_0(y_j) - \frac{\uA}{\cA}\lor\cstar p_0(y_j) = p_0(y_j) - \frac{v}{2}\lor\cstar p_0(y_j)  \geq \frac{1}{2}p_0(y_j)$, so that $\int_{\widetilde C_j}p_0 \geq \frac{1}{2}p_0(y_j) h^d$. Moreover, $p_0^2(x) \leq 2 p_0^2(y_j) + 2 L^2 h^{2\alpha} \lor 2\cstar^2 p_0^2(y_j)  \leq  3 p_0^2(y_j)$. Therefore:
    \begin{align*}
        \int_{\cup_{j \in J_{\text{large}}}} p_0^2 &\leq 3 \sum_{j \in J_{\text{large}}} p_0^2(y_j) h^d = 3 \sum_{j \in J_{\text{large}}} p_0(y_j) h^d \cdot p_0(y_j) h^d \cdot h^{-d}\\
        & \leq 3 \sum_{j \in J_{\text{large}}} 4p_j^2 h^{-d} \leq 12 p_U \sum_{j \geq U} p_j h^{-d} \leq \frac{12c_u}{n^2 h^d}.
    \end{align*}
\end{itemize}
Hence, setting $\CL{\ref{Toute_la_case_OK_moment2}} = \Cmom \lor 12\cu$, we get the result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ¨Cas $Ln < 1$ de la borne triviale

    First case: $Ln \leq 1$. In this case, we prove that if $n \geq n_0$, then $\rhob \geq \rhor$. We first show that if $n\geq \nzero$ and $Ln \leq 1$ then $p_0 \in [1-\cstar , 1+\cstar]$. Indeed, if $n \geq \nzero \geq \frac{L^{\alpha / 2}}{\cstar}$, then denoting by $x \in [0,1]^d$ a point such that $p_0(x) = 1$ (which exists by the intermediate value theorem), we have by Assumption \eqref{simplifyingAssumption} for all $y \in [0,1]^d$: $|p_0(x) - p_0(y)| \leq \cstar \lor L\big(\sqrt{d} \big)^\alpha \leq \cstar$. Now, we show that $|\T(\uA)| \leq \frac{1}{2}$. Indeed, by Lemma \ref{int_p0squared_uA_small} item 2, it holds $n^2 h^d \in [\cI, \Cmom]$ \ju{Définir $|X|$ comme le volume d'un ensemble $X$}.
    \begin{align*}
        (1-\cstar)^2 |\T(\uA)| \leq \int_{\T(\uA)} p_0^2 \leq \frac{\Cmom}{n^2 h^d} = \left(\frac{L^d \left(\int_{\T(\uA)} p_0 \right)^d}{n^{2 \alpha}} \right)^\frac{1}{\alpha + d} \leq \left[\frac{L^d \left((1+\cstar)|\T(\uA)| \right)^d}{n^{2 \alpha}} \right]^\frac{1}{\alpha + d},
    \end{align*}
    \begin{align*}
        \text{hence: } ~~~~ |\T(\uA)| \leq \frac{1}{n^{2\alpha + d}}\frac{(1+\cstar)^\frac{d}{\alpha}}{(1-\cstar)^{\frac{2(\alpha + d)}{\alpha}}} \leq \frac{1}{2}.
    \end{align*}
    \ju{Choisir $n_0$ pour que ce soit vrai: on a besoin de $\frac{1}{n^{2\alpha + d}}\frac{(1+\cstar)^\frac{d}{\alpha}}{(1-\cstar)^{\frac{2(\alpha + d)}{\alpha}}} \leq \frac{1}{2}$ et $\nzero \geq \frac{L^{\alpha / 2}}{\cstar}$} Therefore $|\B| \geq \frac{1}{2}$ so that 
    \begin{align*}
        {\rhob}^t \geq \left(\frac{L^d}{n^{2 \alpha}}  \right)^\frac{t}{4\alpha + d} \left(\frac{1}{2} \right)^\frac{(4-t)\alpha + d}{4\alpha + d} (1-\cstar)^\frac{2\alpha t}{4\alpha + d} =: \left(\frac{L^d}{n^{2 \alpha}}  \right)^\frac{t}{4\alpha + d} \Ccomp.
    \end{align*}
    Now, 
    \begin{align*}
        \frac{{\rhob}^t}{{\rhor}^t} \geq \Ccomp \frac{L^\frac{dt}{4\alpha + d}}{n^\frac{2\alpha t}{4 \alpha + d}} \frac{n^\frac{\alpha t + d}{\alpha + d}}{L^\frac{d(t-1)}{\alpha + d}} \geq n^\frac{2\alpha t}{4 \alpha + d} \text{ using } Ln \leq 1
    \end{align*}
    \ju{Faux !}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]\label{Algo_partitionnement}
\SetAlgoLined
\begin{enumerate}
    \item \textbf{Input:} $\widetilde \Omega, \beta, u, \cbeta$. 
    \item \textbf{Initialization:} $A_0 = \widetilde \Omega$, $~P = \emptyset$, $~\D(u) = \{x \in \widetilde \Omega: p_0(x) \geq u\}$, $~h=\left(\frac{p_0}{\cbeta}\right)^\frac{1}{\beta}$.
    \item For each cube $A_j$: 
        \begin{itemize}
            \item \textbf{If} $A_j \cap \D(u) = \emptyset$ then STOP.
            \item \textbf{Else}:
                \begin{itemize}
                    \item \textbf{If} $e(A_j) \leq h(A_j)$ then do $P \leftarrow P \cup \{A_j\}$; ~ STOP.
                    \item \textbf{Else:} Split $A_j$ into $2^d$ cubes obtained by halving $A_j$ along each of its axes.
                \end{itemize}
        \end{itemize}
    \item Repeat step $3$ on each such defined cube.
    \item \textbf{Return} $P$.
\end{enumerate}
\caption{Adaptive partition}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{align}
    \int_{\widetilde C_j} p^2 \leq \frac{ \AL{\ref{link_2ndMoment__sumSquares}}}{2} \frac{\left(\int_{\widetilde C_j} p \right)^2}{h^d} +2(2+\cstar)^2 L^2(h\sqrt{d})^{2\alpha+d} = \frac{ \AL{\ref{link_2ndMoment__sumSquares}}}{2} \frac{\left(\int_{\widetilde C_j} p \right)^2}{h^d} +2(2+\cstar)^2 d^\alpha  \frac{L h^\alpha}{n\ctail} \label{int_p2}.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{\underline{First case:}} $p(x_j) > \frac{1}{\cstar} Lh^\alpha$. Then by Assumption \eqref{simplifyingAssumption}:
\begin{align*}
    &|p(x) - p_(x_j)| \leq \cstar p(x_j) \Longrightarrow p(x) \in [(1 \pm \cstar)p(x_j)]\\
    \Longrightarrow & \left\{\begin{array}{ll}
         q_j := \int_{\widetilde C_j} p \,\in [(1 \pm \cstar)p(x_j)h^d] \\
         ~~~~~ \int_{\widetilde C_j}p^2 ~~ \in [(1 \pm \cstar)p(x_j)^2 h^d]
    \end{array} \right. \Longrightarrow \left\{\begin{array}{ll}
         p(x_j) \in \left[\frac{1}{1\mp \cstar}\frac{q_j}{h^d}  \right]  \\
         \int_{\widetilde C_j} p^2 \in \left[\frac{1\pm \cstar}{(1 \mp \cstar)^2}\frac{q_j^2}{h^d} \right]
    \end{array} \right.
\end{align*}
hence:
\begin{align*}
    \int_{\widetilde C_j} (p-p_0)^2 \leq 2\int_{\widetilde C_j} p^2 + 2\int_{\widetilde C_j} p_0^2 \leq 2\frac{1 + \cstar}{(1 - \cstar)^2}\frac{q_j^2}{h^d} + 2\int_{\widetilde C_j} p_0^2 \leq 12\frac{q_j^2}{h^d} + 2\int_{\widetilde C_j} p_0^2.
\end{align*}

\textbf{\underline{Second case:}} $p(x_j) \leq \frac{1}{\cstar} Lh^\alpha$. For all $x \in \widetilde C_j$ we have by Assumption \eqref{simplifyingAssumption}:
\begin{align}
    & \left\{\begin{array}{ll}
         p(x) \in [p(x_j) \pm Lh^\alpha] \\
         p_0(x) \in [p_0(x_j) \pm \cstar p_0(x_j) \lor Lh^\alpha]
    \end{array} \right.\nonumber \\
    \text{hence } ~~ & p(x) - p_0(x) \in [p(x_j)-p_0(x_j) \pm 2\cstar p_0(x_j) \lor 2Lh^\alpha]\nonumber \\
    \text{therefore: } ~~ & |p(x) - p_0(x)| \leq |p(x_j) - p_0(x_j)| + 2\cstar p_0(x_j) \lor 2Lh^\alpha \label{abs_p-p0}\\
    \text{and similarly: } ~~ & |p(x_j) - p_0(x_j)| \leq |p(x) - p_0(x)| + 2\cstar p_0(x_j) \lor 2Lh^\alpha \label{abs_p_p0_x_j}
\end{align}
Then for $q_j = \int_{\widetilde C_j}$:\ju{pb reprendre}
\begin{align*}
    \int_{\widetilde C_j} (p-p_0)^2 &\leq \int_{\widetilde C_j}|p-p_0|\big[|p(x_j) - p_0(x_j)| + 2\cstar p_0(x_j) \lor 2Lh^\alpha \big] ~~\text{ by \eqref{abs_p-p0}}\\
    & \leq \int_{\widetilde C_j}|p-p_0| \Big\{\frac{1}{h^d}\int_{\widetilde C_j}|p-p_0| + 4\cstar p_0(x_j) \lor 4Lh^\alpha  \Big\}\\
    & \leq \frac{2}{h^d}\Big(\int_{\widetilde C_j}p \Big)^2 + \frac{2}{h^d}\Big(\int_{\widetilde C_j}p_0 \Big)^2 +  4\cstar p_0(x_j) \lor 4Lh^\alpha \int_{\widetilde C_j}|p-p_0|\\
    &\leq \frac{2}{h^d}q_j^2 + \int_{\widetilde C_j}p_0^2+ 4\cstar p_0(x_j) \lor 4Lh^\alpha \int_{\widetilde C_j}|p-p_0| ~~ \text{ (Cauchy-Schwarz).}
\end{align*}
Moreover: $p_0(x_j) \leq p_0(x) + \cstar p_0(x) \lor L h^\alpha \leq (1+ \cstar)p_0(x) + L h^\alpha$ so that $p_0(x_j) \leq \frac{1+\cstar}{h^d} \int_{\widetilde C_j}p_0 + Lh^\alpha$, hence $p_0(x_j) \int_{\widetilde C_j}|p-p_0| \leq \frac{1+\cstar}{h^d}\big( \int_{\widetilde C_j}p_0\big)^2 + \frac{1+\cstar}{h^d}q_j \int_{\widetilde C_j}p_0 + Lh^\alpha \int_{\widetilde C_j}|p-p_0|$:
\begin{align*}
    \int_{\widetilde C_j} (p-p_0)^2 &\leq \frac{2q_j^2}{h^d} + (2+\cstar) \int_{\widetilde C_j}p_0^2+ 4(1+\cstar)Lh^\alpha \int_{\widetilde C_j}|p-p_0| + \frac{\cstar(1+ \cstar)}{h^d}q_j\int_{\widetilde C_j}p_0\\
    & \leq \frac{2\cstar(1 + \cstar) q_j^2}{h^d} + (2+2\cstar +\cstar^2) \int_{\widetilde C_j}p_0^2 + 4(1+\cstar)Lh^\alpha \int_{\widetilde C_j}|p-p_0|\\
    &\leq \frac{3q_j^2}{h^d} + 4\int_{\widetilde C_j}p_0^2 + 6Lh^\alpha \int_{\widetilde C_j}|p-p_0|.
\end{align*}
\ju{Vérifier pour les constantes}



The result is obtained by summing over $j=1,\dots, M$ and recalling that, by lemma \ref{int_p0squared_uA_small}, $\int_{\T(\uA)} p_0^2 \leq \Cmom \frac{1}{n^2\barhT^d} \leq \Cmom \frac{1}{n^2\hT^d(\uA)}$, no matter whether $\uA = \uI$ or $\uA > \uI$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There are two cases:
\begin{itemize}
    \item First case: $\cstar p(x), \cstar p(y) \leq L\|x-y\|^\alpha$. Then by Assumption \eqref{simplifyingAssumption},
    \begin{align*}
        |p(x) + \phi(x) - p(y) - \phi(y)| &\leq |p(x) - p(y)| + |\phi(x)| + |\phi(y)| \leq  L \|x-y\|^\alpha + c(p(x) + p(y))\\
        & \leq \left(1 + \frac{2c}{\cstar} \right) L \|x-y\|^\alpha \leq \left(1 + \frac{2c}{\cstar} \right) \left[ \cstar p(x) \lor L \|x-y\|^\alpha\right].
    \end{align*}
    \item Second case: $\cstar(p(x) \lor p(y)) > L\|x-y\|^\alpha$. Then by \eqref{simplifying_assumpt_satisfied}, assuming $p(x) \geq p(y)$ by symmetry, we have $|p(x) - p(y)| \leq \cstar p(x)$ hence $p(y) \geq (1-\cstar )p(x)$. Therefore:
    \begin{align*}
        |p(x) + \phi(x) - p(y) - \phi(y)| &\leq \cstar p(x) + c(p(x) + p(y)) \leq \left(1 + \frac{2c}{\cstar} \right) \left[ \cstar p(x) \lor L \|x-y\|^\alpha\right].
    \end{align*}
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pour borne inf bulk : cases incluses dans B(uA/2)

\begin{lemma}\label{cubesBulk_geq_uA/2}
For all $j=1, \dots, N : \inf_{B_j}p_0 \geq \frac{\uA}{2}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{cubesBulk_geq_uA/2}]
Fix $j \in \{1,\dots, N\}$. By definition of the splitting, $B_j \cap \B \neq \emptyset$ and the edge length of $B_j$ is at most $h_j = c \hB(x_j)$ where $x_j$ is the center of $B_j$. Let $z_j = \arg \max_{B_j \cap \B} \, p_0$. For all $x \in B_j$ we have by Assumption \eqref{simplifyingAssumption}:
\begin{align*}
    |p_0(x) - p_0(z_j)| &\leq \cstar p_0(z_j) + L(h_j \sqrt{d})^\alpha  \leq \Big(\cstar + \frac{c}{\cA}  \Big) p_0(z_j) \leq \frac{p_0(z_j)}{2},
\end{align*}
since $h_j \sqrt{d} = c\hB(x_j)\sqrt{d} \leq c\hB(x_j) \leq c\hB(z_j)$ and $L \hB(z_j)^\alpha \leq \frac{p_0(z_j)}{\cA}$. Therefore, $p_0(x)\geq \frac{p_0(z_j)}{2} \geq \frac{\uA}{2}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

By direct calculation, we have for any constant $C>0$:
\begin{align*}
    {\rhob}^t \geq C{\rhot}^t \Longrightarrow \uA^{2-r} \I \geq  \frac{C(\uA)}{n^2 \hT^d(\uA)}  
\end{align*}
where $C(\uA) $ is an absolute constant depending only on  $C$ and $\uA$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    If $x \in \D(u)$ then $p_0(x) \geq \frac{u}{2}$ by definition of $\D(u)$. Suppose that $x \in \cup_{A \in P} A \setminus \D(u)$. Let $j \in \{1,\dots,M\}$ such that $x \in B_j$ and $y \in \arg\max_{B_j \cap \D(u)} p_0$. We have by Proposition \ref{guarantees_algo} item 2 $e(A_j) \leq h(A_j) \leq h(y)$ so that by Assumption \eqref{simplifyingAssumption}:
    \begin{align*}
        p_0(x) &\geq (1-\cstar) p_0(y) -L(e(A_j)\sqrt{d})^\alpha \\
        &\geq (1-\cstar) p_0(y) -L(h(y)\sqrt{d})^\alpha \\
        & \geq (1-\cstar) p_0(y) -\sqrt{d}^\alpha \frac{1}{\calpha} p_0(y)\\
        &\geq \frac{u}{2} ~~ \text{by definition of }\calpha.
    \end{align*}
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{norm_gammaup_geq_normp0}
For all $j\geq U$ it holds $\|\gammaup_j\|_t^t \geq \frac{\Cintt}{\Cmom} \|p_0\|_t^t$ where $\Cintt = \int_{\R^d} (1-\|x\|)_+^{\alpha t} dx$.
\end{lemma}
\begin{proof}
By the definition of $\gammaup_j$ \eqref{def_gamma} we have:
\begin{align*}
    \|\gammaup_j\|_t^t &= \Cintt L^t h^{\alpha t + d} = \Cintt (\rhot)^t \geq \left(\int_{\T(\uA)} p_0 \right) \left(Lh^{\alpha +d} \frac{1}{n^2 h^d}\right)^{t-1} \\
    & \geq \Cintt \left(\int_{\T(\uA)} p_0 \right)^{2-t} \left(\frac{1}{\Cmom} \int_{\T(\uA)} p_0^2 \right)^{t-1} ~~ \text{ by Lemma \ref{int_p0squared_uA_small}}\\
    & \geq \frac{\Cintt}{\Cmom^{t-1}} \|p_0\|_t^t ~~ \text{ by Hölder's inequality, which proves the lemma.}
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Moreover,  by lemma \ref{gammadown_lesssim_intp0}, for all $j \geq U$: $\frac{\Gammadown_j}{\Gammaup_j} \leq \frac{\Cint \cdown p_j n^2 \sum_{j\geq U} p_j}{\Cint \cupward_j} \leq \frac{\cu \cdown}{\cupward} \leq \Cint \cdown /\Cdown = \frac{\cu}{(1-\cstar)} \leq 2 \cu $, recalling that $\forall j\geq U: \cupward_j \in \left[\frac{\cu \Cdown}{\Cint}, \frac{2\cu \Cdown}{\Cint} \right]$. Therefore:
\begin{align*}
    \mathbb{V}[\|q_b\|_1] &\leq \sum_{j \geq U} \pi_j \left(1 + 2 \cu \right)^2 {\Gammaup_j}^2 \leq \sum_{j \geq U} \pi_j \left(1 + 2\cu \right)^2 \left[\cupward_j \frac{\Cint}{n^2 \sum_{j' \geq U} p_{j'}}\right]^2\\
    & \leq \left(1 + 2\cu \right)^2 \left[\frac{2\cu \Cdown}{\Cint}\right]^2 \Cint^2 \frac{n^2 \big(\sum_{j\geq U} p_j\big)^2}{\cu} \frac{1}{n^4\big(\sum_{j\geq U} p_j\big)^2}\\
    & \leq (1 + 2 \cu)^2 4 \cu \Cint^2 \frac{1}{n^2}.
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{pU_small_sum_large}
There exists an absolute constant $D$, % $D = \frac{\cu}{6\Cstep}$ \ju{A modifier}
such that whenever $\int_{\T(\uA)} p_0 \geq \frac{\ctail}{n}$ and $p_U \leq \Cstep L h^{\alpha+d}$, it holds: $\sum_{j\geq U} p_j \geq D \int_{\T(\uA)} p_0$. Moreover, $D$ \ssmall{$\cu$} and $\ctail$ large enough.
\end{lemma}

%\ju{On a besoin de $\ctail^2 \geq \frac{18 \Cstep^2}{\cu}$. A modifier aussi ! Ce n'est plus la bonne constante}

\begin{proof}[Proof of Lemma \ref{pU_small_sum_large}]
If $U=1$ then since $\T(\uA) \subset \bigcup\limits_{j=1}^M \widetilde C_j$, we have $\sum\limits_{j\geq U} p_j \geq \int_{\T(\uA)} p_0$ hence the result is clear. Assume now that $U \geq 2$ and that $p_U \leq 2\Cmom L h^{\alpha + d}$. We can then write, by definition of $U$:
\begin{align*}
    p_{U-1} \sum_{j \geq U-1} p_j > \frac{\cu}{n^2},
\end{align*} where $p_{U-1} \leq \Cstep' L h^{\alpha+d}$ by Lemma \ref{only_small_jumps}, and $\Cstep' = (2+\cstar) \Cstep$. Therefore:
\begin{align*}
    \sum_{j \geq U} p_j &> \frac{\cu}{n^2 p_{U-1}} - p_{U-1} \geq \frac{\cu}{n^2 \Cstep' L h^{\alpha + d}} - \Cstep' L h^{\alpha + d}\\
    & = \frac{\cu}{\Cstep'} \int_{\T(\uA)} p_0 - \frac{\Cstep'}{n^2 \int_{\T(\uA)} p_0}\\
    & \geq \frac{\cu}{\Cstep'} \int_{\T(\uA)} p_0 - \frac{\Cstep'}{\ctail^2} \int_{\T(\uA)} p_0\geq D \int_{\T(\uA)} p_0.
\end{align*}
Choosing $\ctail^2 \geq \frac{\Cstep'^2}{2\cu}$ yields the result with $D = \frac{\cu}{\Cstep'} - \frac{\Cstep'}{\ctail^2}$.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Ancienne preuve du lemme \ref{Toute_la_case_OK_moment1}
%and $v := \frac{4}{\cA}\uA$. 
\begin{itemize}
    \item \underline{First case}: $p_U \geq \frac{v}{4} h^d$. Then
    \begin{align*}
        p_U \geq \frac{1}{\cA}\uA h^d \geq  L \inf_\B \hB^\alpha h^d \geq  L h^{\alpha + d} =  \frac{1}{n^2 \int_{\T(\uA)} p_0}.
    \end{align*} Moreover, we have by definition of $U$: $\sum_{j \geq U} p_j \leq \frac{\cu}{n^2 p_U}$, so that $\sum_{j \geq U} p_j \leq \cu \int_{\T(\uA)} p_0.$ 
    \item \underline{Second case}: $p_U < \frac{v}{4} h^d$. Then $\forall j \geq U: p_j < \frac{v}{2} h^d$ since $p_U \geq \dots \geq p_M$. By Lemma \ref{very_small_p_0} we therefore have $p_0 < v < \uA$ on $\widetilde C_U$ since $4 < \cA$ \ju{A prendre en compte}. Therefore, $\widetilde C_j \subset \T(\uA)$ for all $j \geq U$, which proves $\sum_{j \geq U} p_j \leq \int_{\T(\uA)} p_0$. 
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Overview
We fix $p_0 \in \mathcal{P}(\alpha, L)$ defined in \eqref{class_densities}, along with some constant $\eta \in (0,1)$. We first give an overview of our results. The domain $\Omega = [0,1]^d$ will be split into two parts. On the one hand, the \textit{bulk} part, where $p_0$ takes only large values:
\begin{equation}\label{def_Bulk}
    \B = \{x\in \Omega: p_0(x) \geq \uA\},
\end{equation} for some value $\uA$ to be defined later on. On the other hand, the \textit{tail}, where $p_0$ takes only small values:
\begin{equation}\label{def_tail}
    \mathcal{T} = \B^c = \{x\in \Omega: p_0(x) < \uA\}.
\end{equation}
The analysis will be divided into two parts. The first part will be concerned with the bulk; the second one with the tail. In each case, we will restrict $p_0$ to each particular set, and establish the minimax separation radii $\rhob$ and $\rhot$ separately. Likewise, we will identify the optimal tests $\psib$ and $\psit$ independently on each set. The overall minimax separation radius $\eqref{separation_radius}$ will be given - up to absolute multiplicative constants - by the sum of the two terms: $\rho^* \asymp \rhob + \rhot$, and the overall optimal test by the combination of the two tests: $\psi^* = \psib \lor \psit$. \ju{Très redondant avec la suite}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Therefore:
\begin{equation}\label{Majorant_JDc}
    J_{\D^c} \leq \left(\frac{12\CK^4}{n^2} + \frac{96 \CK^2}{n\sqrt{\cp}} + \frac{200}{\cp}\right) t_n^2 + \frac{96 \CK^2}{n^2} t_n J + \frac{200}{n^2}J^2.
\end{equation}
\ju{Adapter ce majorant}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% B(uI) = B(uA)

\begin{lemma}\label{I(uA)=I(uI)}
There exists an absolute constant $\CL{\ref{I(uA)=I(uI)}}$ such that $\int_{\B(\uA)} p_0^r \geq \CL{\ref{I(uA)=I(uI)}} \int_{\B(\uI)} p_0^r = \CL{\ref{I(uA)=I(uI)}} \I$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{I(uA)=I(uI)}]
If $\uI = \uA$, then the result is clear. Now, suppose $\uI < \uA$. Then it holds:
\begin{align*}
     \I \uA^{2-r} &~\leq~ \frac{\CL{\ref{tail_dominates}}}{n^2} \frac{\barhT^{{d^2/\alpha}}}{\hT^{d(\alpha+d)/\alpha}} \hspace{15mm} \text{ by Lemma \ref{tail_dominates}}\\
     &~\leq~ \frac{\CL{\ref{tail_dominates}} \; \CL{\ref{htail_all_equal}}^{d^2/\alpha}}{n^2 \hT^d} \hspace{21mm} \text{ by Lemma \ref{htail_all_equal}}\\
     & ~\leq~ \frac{\CL{\ref{tail_dominates}} \; \CL{\ref{htail_all_equal}}^{d^2/\alpha}}{\cI} \int_{\B(\uA)} \hspace{-5mm} p_0^2  \hspace{11mm} \text{ by definition of $\uI$ and recalling $\uA>\uI$}\\
     & ~\leq~ \frac{\CL{\ref{tail_dominates}} \; \CL{\ref{htail_all_equal}}^{d^2/\alpha}}{\cI} \uA^{2-r} \int_{\B(\uA)} \hspace{-5mm} p_0^r,
\end{align*}
hence the result is obtained with $\CL{\ref{I(uA)=I(uI)}} := \frac{\cI}{\CL{\ref{tail_dominates}} \; \CL{\ref{htail_all_equal}}^{d^2/\alpha}}$ which is an absolute constant.
\ju{La fin de cette preuve ça veut pas dire qu'on n'a pas du tout besoin de $\B(\uI)$ finalement ?}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theoreme UB tail

\begin{itemize}
    \item Whenever the tail dominates, i.e. when $\rhot \geq \CBT \rhob$, it holds: $$ \mathbb{P}_{p_0}(\psit=1) + \sup\limits_{p \in \mathcal{P}_{Tail}(\ThreshT\rhot)} \mathbb{P}_p(\psit=0) \leq \frac{\eta}{2}.$$
    \item Whenever the bulk dominates, i.e. when $\rhob \geq \CBT \rhot$, it holds: $$ \mathbb{P}_{p_0}(\psit=1) + \sup\limits_{p \in \mathcal{P}_{Tail}(\ThreshT\rhob)} \mathbb{P}_p(\psit=0) \leq \frac{\eta}{2}.$$
\end{itemize}
%There exists a constant  such that $R(\psit, \ThreshT \rhot)\leq \eta. $


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Disjonction de cas pour borne inf tail (corps du texte)

\underline{\textbf{First case}}: $\int_{\T} p_0 \leq \frac{\ctail}{n}$ where $\ctail$ is a large absolute constant.  %\ju{Il semblerait qu'il vaille mieux discuter selon la valeur de $\int_{\T(\uI)} p_0$ : si elle est $\geq \frac{\ctail}{n}$ alors $\int_{\T(\uA)}p_0$ aussi.} 
In this case we set the prior given in Equation \eqref{prior_remainder} and we get the following lower bound:


\vspace{3mm}

\underline{\textbf{Second case}}: $\int_{\T} p_0 > \frac{\ctail}{n}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Faux lemme borne triviale

\begin{lemma}\label{uI_geq_max_p0}
If $\uI > \max\limits_\Omega p_0$ then $\rho^* \asymp \TL^\frac{t-1}{\alpha+d}$. This corresponds to the trivial rate (namely the $\ell_t$ diameter of $\mathcal{P}(\alpha,L',\cstar')$).
\end{lemma}

\begin{proof}[Proof of Lemma \ref{uI_geq_max_p0}]
If $\uI > \max\limits_\Omega p_0$ then we have: $\uA > \max\limits_\Omega p_0$, $\rhob = 0$, hence the tail dominates. Moreover $\int_{\T(\uA)} p_0 = 1 \geq \frac{\ctail}{n}$ for $n$ large enough. Therefore, by Proposition \ref{Lower_bound_tail_proposition}, $\rho^* \geq \CtailLB \rhot = \CtailLB \TL^\frac{t-1}{\alpha+d}$. Lemma \ref{control_norm_t_Rd} yields the matching upper bound. Since any density $p\in \mathcal{P}(\alpha,L',\cstar')$ has $\ell_t$ norm upper bounded by $\BL{\ref{control_norm_t_Rd}}$, this corresponds to the trivial rate.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Locality of the results}

For fixed dimensionality $d$ of the ambient space $\R^d$, we provide an example of a sequence of null densities $(\pzeron)_{n \in \N}$ and $(L_n)_n$ a sequence of nonnegative numbers such that the local detection threshold $\rho^*\big(p_0^{(n)}, n , L_n\big)$ satisfies $\rho^*\big(p_0^{(n)}, n, L_n\big) = o\big(\rho^*\big(\mathbb{1}_{[0,1]^d}, n, L_n\big)\big)$.\\

Assume $t=1$, $d=1$ and $\alpha = 1$. In other words, we consider the problem of testing in total variation distance against Lipschitz alternatives. Set for all $n \in \N$: $L_n = n$ and $\pzeron = n - L_n\big(\frac{1}{n} - |x|\big)_+$

\hfill

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Relations entre constantes

\ju{Je mets ici les conditions que doivent remplir les constantes pour pouvoir tunées quand toute la preuve sera écrite :
\begin{itemize}
    \item On a besoin de $\Cmom \leq \frac{\eta}{4}$ cf errI de $\psi_2$.
    \item On a besoin de $c_u \geq 2\cI$ mais en fait il se peut qu'on ait pas du tout besoin de $\cu$.
    \item $\cI \leq 1$ pour que $\lambda \leq 1$.
    \item on a besoin de $\RadB \geq 1$ pour que l'espérance de $\mathbb E \Tb \gtrsim$ sous H1.
    \item On a besoin que $\cstar + \frac{2}{\calpha} \left(\frac{\sqrt{d}}{2} \right)^\alpha \leq 1/2$ dans l'analyse de l'algo. %De plus pour le lemma \ref{cubesBulk_geq_uA/2} : $\cstar + \frac{c}{\cA} \leq \frac{1}{2}$. A-t-on vraiment besoin du lemme \ref{cubesBulk_geq_uA/2} ?
    \item On a besoin de $\frac{\Cmom}{\Cstep} < 1$ pour le lemme \ref{very_small_dominate}
    \item On a besoin de $\ctail^2 \geq \frac{18 \Cstep^2}{\cu}$ pour le lemme \ref{sum_pj_geq_int}.
    %\item On a besoin de $c \leq \frac{1}{\sqrt{d}}$ cf Lemme \ref{cubesBulk_geq_uA/2}.
    \item On peut ajuster $\Cmom$ pour que $D \leq \big(1-\frac{\Cmom}{\Cstep} \big)$ dans le Lemme \ref{sum_pj_geq_int}.
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Extension to nonbounded domain

\section{Extension to non bounded domain}

We now show how our analysis for densities on $[0,1]^d$ can be transferred to handle the case of densities on $\R^d$. By convention, we consider $\R^d$ as a cubic domain of $\R^d$. Note that any density defined over a bounded cubic domain in $\R^d$ can be modified through translation and rotation to get a density over $[0,\lambda]^d$ for some $\lambda>0$. We consider $d$ and $t$ as being fixed. Introduce, for any cubic domain $\Omega' \subset \R^d$:
\begin{align}
    %\forall a < b: \mathcal{P}_{a,b}(\alpha,L,\cstar) &= \left\{p\text{  density over } [a,b]^d ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $[a,b]^d$} \right\}, \label{def_P_ab}\\
     \mathcal{P}_{\Omega'}(\alpha,L,\cstar) &= \left\{p\text{  density over } \Omega' ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $\Omega'$} \right\}, \label{def_P_cubic}
\end{align}
If $\Omega'$ is of the form $[0,\lambda]^d$ for $\lambda>0$, we denote for simplicity $\mathcal{P}_{\Omega'}(\alpha,L,\cstar)$ by $\mathcal{P}_\lambda(\alpha,L,\cstar)$.
%$\forall \lambda>0: \mathcal{P}_\lambda(\alpha,L,\cstar) &= \left\{p\text{  density over } [0,\lambda]^d ~\big|~ p\in H(\alpha,L) \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $[0,\lambda]^d$} \right\}, \label{def_P_H}\\$
Fix $\lambda_1, \lambda_2>0$ and $\lambda=\lambda_1/\lambda_2$. Define the rescaling operator:
\begin{equation}\label{rescaling_operator}
    \Phi_{\lambda_1,\lambda_2}: \left\{ \begin{array}{ccc}
        \mathcal{P}_{\lambda_1}(\alpha,L,\cstar) & \longrightarrow & \mathcal{P}_{\lambda_2}(\alpha, L \lambda^{\alpha+d},\cstar)\\
        &&\\
        p & \mapsto & \lambda^d\, p(\lambda \, \cdot \,) 
    \end{array}\right. 
\end{equation}
where $p(\lambda \, \cdot \,) : x \mapsto p(\lambda x)$. We show in Lemma \ref{Rescaling} that $\Phi_{\lambda_1,\lambda_2}$ is the natural operator for transferring the rates over $[0,\lambda_1]^d$ to $[0,\lambda_2]^d$. For any cubic domain $\Omega' \subset \R^d$, we define $\rho_{\Omega'}^*(p_0,\alpha,L,n)$ as the minimax separation radius for the following testing problem over $\Omega'$, upon observing $X_1,\dots,X_n$ iid with density $p \in \mathcal{P}_{\Omega'}(\alpha,L,\cstar)$ 


%For fixed $\lambda>0$ and for $p_0 \in \mathcal{P}_\lambda(\alpha,L,\cstar)$ (resp. $p_0 \in \mathcal{P}_{\R^d}(\alpha,L,\cstar)$), define $\rho_\lambda^*(p_0,\alpha,L,n)$ (resp. $\rho_{\R^d}^*(p_0,\alpha,L,n)$ ) as the minimax separation radius for the following testing problem over $[0,\lambda]^d$ (resp. $\R^d$), upon observing $X_1,\dots,X_n$ iid with density $p \in \mathcal{P}_\lambda(\alpha,L,\cstar)$ (resp. $\mathcal{P}_{\R^d}(\alpha,L,\cstar)$):
\begin{align}\label{testing_pb_lambda}
\begin{split}
    H_0~~~ &: \; p = p_0 \;\;~~~~~~\; \text{ versus }\\
    H_1^{(\Omega')}(\rho) &:\; p \in \mathcal{P}_{\Omega'}(\alpha,L', \cstar') ~ \text{ s.t. } \norm{p-p_0}_t \geq \rho.
\end{split}
\end{align}
Similarly, if $\Omega'$ is of the form $[0,\lambda]^d$ for $\lambda>0$, we denote for simplicity $\rho_{\Omega'}^*(p_0,\alpha,L,n)$ by $\rho_\lambda^*(p_0,\alpha,L,n)$.
We now state the following Proposition, guaranteeing that our analysis over $[0,1]^d$ can be transferred, by homogeneity, to densities on any bounded cube $[0,\lambda]^d$ for $\lambda>0$, and by translation and rotation, to any cubic domain in $\R^d$. 

\begin{proposition}\label{transfer_rate}(Rescaling)
Let $\lambda_1, \lambda_2>0$ and $\lambda = \lambda_1/\lambda_2$ and let $p_0 \in \mathcal{P}_{\lambda_1}(\alpha,\, L,\,\cstar)$. It holds
$$ \rho_{\lambda_2}^*\left(\Phi_{\lambda_1,\lambda_2}(p_0),\, \alpha,\, L\lambda^{\alpha+d},\, n\right) = \lambda^{\frac{d}{t}-d}\,\rho_{\lambda_1}^*\left(p_0, \alpha, L, n \right).$$
\end{proposition}

We can now analyze the unbounded case. The following Proposition states that the unbounded case can be deduced from the bounded case by restricting the density to a sufficiently large bounded cubic domain $\Omega'$ (in the sense that the total mass of $p_0$ outside $\Omega'$ is at most $O(1/n)$.) Moreover, an optimal test on $\R^d$ can be obtained by combining any optimal test on $\Omega'$ with the test rejecting $H_0$ whenever at least one of the observations $(X_i)_i$ belongs to $\R^d \setminus \Omega'$.\\

Let $p_0 \in \mathcal{P}_{\R^d}(\alpha,L,\cstar)$. Set $\lambda>0$ such that $V:= \int_{[-\lambda,\lambda]^d}p_0 \geq 1- \frac{\cRd}{n}$ for some absolute constant $\cRd$ sufficiently small. Define $\Omega' = [-\lambda,\lambda]^d$ and $$\barpzero : \Omega' \longrightarrow \R_+; ~ x\mapsto \frac{1}{V}p_0(x).$$ 
For all $\rho>0$, define
\begin{equation}\label{def_P_omega_rho}
    \mathcal{P}_{\Omega'}(\rho) = \{p \in \mathcal{P}_{\Omega'}(\alpha, L,\cstar) : \|p-\barpzero\|_t \geq \rho\}.
\end{equation}
For any test $\psi$ and all $\rho>0$, define the risk of $\psi$ with radius $\rho$ on $\Omega'$:
\begin{equation}\label{risk_Omega'}
    R_{\Omega'}(\psi, \rho) =  \mathbb{P}_{\barpzero}(\psi=0) + \sup_{p \in \mathcal{P}_{\Omega'}(\rho)} \mathbb{P}_p(\psi=1) .
\end{equation}

\begin{proposition}\label{unbounded_case}(Unbounded case)
It holds: $$\rho_{\R^d}^*(p_0, L,n) \asymp \rho_{\Omega'}^*(\barpzero, L,n).$$
Moreover, if $\barpsistar$ is a test satisfying $R_{\Omega'}(\barpsistar, C\rho_{\Omega'}^*(\barpzero, L,n)) \leq \frac{\eta}{2}$ for some absolute constant $C$ sufficiently large, then, for $\psi^* := \barpsistar \lor \mathbb{1}\left\{\bigvee\limits_{i=1}^n (X_i \notin \Omega')\right\}$, we have: $R_{\R^d}(\barpsistar, C'\rho_{\Omega'}^*(\barpzero, L,n)) \leq \eta$ for some absolute constant $C'$ sufficiently large.
%Moreover, for all $\rho>0$ define $\mathcal{P}_{\Omega'}(\rho) = \{p \in \mathcal{P}_{\Omega'}(\alpha, L,) : \|p-\barpzero\|_t \geq \rho\}$. 

\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Extension non bounded domain proofs

\section{Extension to unbounded domains}\label{Extension_unbounded_domains}

For any prior distribution $\pi$ over $\mathcal{P}_\lambda(\alpha,L,\cstar)$ (i.e. such that $\int_{\mathcal{P}_\lambda(\alpha,L,\cstar)} d\pi = 1$) we denote by $\widetilde \pi$ the probability measure induced by $\pi$ over $([0,\lambda]^d)^n$:
$$\forall A \subset ([0,\lambda]^d)^n \text{ measurable, } \widetilde \pi(A) = \int_{\mathcal{P}_\lambda(\alpha,L,\cstar)}\hspace{-5mm} p(A) d\pi(p).$$ 

\begin{lemma}\label{Rescaling}
For all $\lambda_1,\lambda_2>0$, let $\lambda = \lambda_1/\lambda_2$. We have the following guarantees:
\begin{enumerate}
    \item $\Phi_{\lambda_1,\lambda_2}$ is well-defined and bijective.
    \item For all $p,q \in \mathcal{P}_{\lambda_1}(\alpha,L,\cstar)$: $\|\Phi_{\lambda_1,\lambda_2}(p) - \Phi_{\lambda_1,\lambda_2}(q)\|_t = \lambda^{d-d/t}\|p-q\|_t$.
    \item $d_{TV}(\widetilde \pi, p_0^{\otimes n}) = d_{TV}(\widetilde{\Phi_{\lambda_1,\lambda_2}}(\pi), \Phi(p_0)^{\otimes n})$.
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Rescaling}]
\begin{enumerate}
    \item We first check that $\Phi_{\lambda_1, \lambda_2}$ is well-defined. For all $x,y \in [0,\lambda_2]^d$, for all $p \in \mathcal{P}_{\lambda_1}(\alpha, L, \cstar)$ we have for $m:= \lceil \alpha-1 \rceil$:
    \begin{align*}
        \left|\Phi_{\lambda_1, \lambda_2}(p)^{(m)}(x)-\Phi_{\lambda_1, \lambda_2}(p)^{(m)}(y)\right| \leq \lambda^d \lambda^m \left|p^{(m)}(\lambda x) - p^{(m)}(\lambda y)\right|^{\alpha - m} \leq \lambda^{\alpha + d} L \|x-y\|^{\alpha - m},
    \end{align*}
    so that $\Phi_{\lambda_1, \lambda_2}(p) \in H(\alpha, L \lambda^{\alpha+d})$. Moreover, by Assumption \eqref{simplifyingAssumption}:
    \begin{align*}
        \left|\Phi_{\lambda_1, \lambda_2}(p)(x) - \Phi_{\lambda_1, \lambda_2}(p)(y)\right| &= \lambda^d|p(\lambda x) - p(\lambda y)| \leq \cstar \lambda^d p(\lambda x) + L \lambda^d\|\lambda x - \lambda y\|^\alpha\\
        & = \cstar \Phi_{\lambda_1, \lambda_2}(p)(x) + L \lambda^{\alpha + d}\|x-y\|^\alpha,
    \end{align*}
    hence $\Phi_{\lambda_1, \lambda_2}(p)$ satisfies Assumption \eqref{simplifyingAssumption} over $[0,\lambda_2]^d$ with the constants $\cstar$ and $L \lambda^{\alpha+d}$. It follows that $\Phi_{\lambda_1, \lambda_2}(p)$ is well-defined. Moreover, 
    the application $\Phi_{\lambda_1, \lambda_2}$ is clearly invertible since $\Phi_{\lambda_1, \lambda_2}\circ\Phi_{\lambda_2, \lambda_1} = \text{Id}_{\,\mathcal{P}_{\lambda_1}(\alpha, L, \cstar)}$, and $\Phi_{\lambda_2, \lambda_1}\circ\Phi_{\lambda_1, \lambda_2} = \text{Id}_{\,\mathcal{P}_{\lambda_2}(\alpha, L\lambda^{\alpha+d}, \cstar)}$ hence bijective.
    \item Fix $p,q \in \mathcal{P}_{\lambda_1}(\alpha, L, \cstar)$. We have:
    \begin{align*}
        \|\Phi_{\lambda_1, \lambda_2}(p)-\Phi_{\lambda_1, \lambda_2}(q)\|_t^t = \int_{[0,\lambda_2]^d} \hspace{-5mm} \lambda^{t d} \left|p(\lambda x) - q(\lambda x)\right|^t dx = \lambda^{td - d} \|p-q\|_t^t.
    \end{align*}
    \item For all prior $\pi$ over $\mathcal{P}_{\lambda_1}(\alpha,L,\cstar)$, $\widetilde \pi$ is absolutely continuous w.r.t. the Lebesgue measure over $([0,\lambda_1]^d)^n$. We therefore have:
    \begin{align*}
        d_{TV}(\widetilde \pi, p_0^{\otimes n}) &= \frac{1}{2} \int_{([0,\lambda_1]^d)^n} \left|\widetilde \pi(x) - p_0^{\otimes n}(x)\right|dx = \frac{1}{2} \int_{([0,\lambda_2]^d)^n} \left|\widetilde \pi(\lambda y) - p_0^{\otimes n}(\lambda y)\right| \lambda^{nd}dy \\
        & = \frac{1}{2} \int_{([0,\lambda_2]^d)^n} \left|\widetilde{\Phi_{\lambda_1, \lambda_2}(\pi)}(y) - \Phi_{\lambda_1,\lambda_2}(p_0)^{\otimes n}(y)\right|dy\\
        & = d_{TV}(\widetilde{\Phi_{\lambda_1, \lambda_2}(\pi)}, \Phi_{\lambda_1,\lambda_2}(p_0)^{\otimes n}).
    \end{align*}
\end{enumerate}
\end{proof}

\subsection{Proof of Proposition \ref{transfer_rate}}

\hfill

\begin{proof}[Proof of Proposition \ref{transfer_rate}]
It holds: \ju{A compléter !!!}
\begin{align*}
    \rho_{\lambda_1}^*(p_0, \alpha, L, n) = \sup \left\{ \|\pi - p_0\|_t \right\}
\end{align*}
\end{proof}

\subsection{Proof of Proposition \ref{unbounded_case}}


\begin{proof}[Proof of Proposition \ref{unbounded_case}]

\hfill

\underline{\textbf{Lower bound:}} ($\rho_{\R^d}^*(p_0, L,n) \gtrsim \rho_{\Omega'}^*(\barpzero, L,n)$).\\

For any cube $K$ and any density $q$ over $K$, define
\begin{align}
    H_{K}(\alpha,L,\cstar) &= \left\{p \in H(\alpha, L) ~|~ p\geq 0 \text{ and $p$ satisfies \eqref{simplifyingAssumption} over $K$} \right\}\\
    \mathcal{P}_{K}(q, \alpha,L,\cstar) &= \left\{p \in H_{K}(\alpha,L,\cstar) ~\big|~ p=q \text{ on } \partial K \right\}.\label{def_P_boundaries}
\end{align}
If $K = [0,\lambda]^d$, we simply write $\mathcal{P}_{\lambda}(q, \alpha,L,\cstar)$. Note that in our analysis of the case $[0,1]^d$ we guarantee that for all $q_0 \in \mathcal{P}_1(\alpha, L, \cstar)$, our bulk prior \eqref{prior_bulk} and remainder prior \eqref{prior_remainder} have support in $\mathcal{P}_1(q_0,\alpha, L, \cstar)$. Our tail prior \eqref{def_prior_tail}, however, does not have support on $\mathcal{P}_1(q_0,\alpha, L, \cstar)$. We therefore analyse these two cases separately. By homogeneity (see Proposition \ref{transfer_rate}), assume \textit{wlog} that $\Omega' = [0,1]^d =\Omega$. In both cases, we will take a prior distribution over $\Omega'$ and transform it into a prior distribution over $\R^d$. This is done through the following transformation:
\begin{equation}\label{def_transfer_prior}
    \Theta : \left\{\begin{array}{ccl}
         \mathcal{P}_1(\barpzero, \alpha, \frac{L}{p_0(\Omega)}, \cstar) & \longrightarrow & \mathcal{P}_{\R^d}(\alpha,L,\cstar) \\
         p & \mapsto & p_0(\Omega)\; \mathbb{1}_\Omega \; p + \mathbb{1}_{\R^d \setminus \Omega}\; p_0
    \end{array}\right.
\end{equation}
where $p_0(\Omega) = \int_{\Omega}p_0$. For any prior distribution $\pi$ over $\mathcal{P}_1(\barpzero, \alpha, \frac{L}{p_0(\Omega)}, \cstar)$, we denote by $\Theta(\pi)$ the image probability measure of $\pi$ by $\Theta$, defined as: $\Theta(\pi)(A) = \pi(\Theta^{-1}(A))$ for all $A \subset \mathcal{P}_{\R^d}(\alpha,L,\cstar)$ measurable. Define also 
\begin{equation}\label{def_Aout}
    \Aout = \left\{\forall i=1, \dots, n: X_i \in \Omega'\right\}.
\end{equation}
Then, $\mathbb{P}_{p_0}\left(\Aout^c\right) = \mathbb{P}_{\Theta(\pi)}\left(\Aout^c\right) \leq \cRd$ by a union bound, so that $\Aout$ can have arbitrarily large probability provided $\cRd$ is small enough, i.e. $\lambda$ is large enough.\\

The density $\barpzero$ will play the role of the null density over $\Omega$. We first consider the cases where $\pi$ is defined as in \eqref{prior_bulk} or in \eqref{prior_remainder} with $\barpzero$ instead of $p_0$. In these cases, we can write:
\begin{align*}
    d_{TV}(\widetilde{\Theta(\pi}), p_0^{\otimes n}) & \leq \sup_{A} \left|\widetilde{\Theta(\pi})(A) - p_0^{\otimes n}(A)\right|\mathbb{P}_{p_0}\left(\Aout\right) + 2 \cRd\\
    &= d_{TV}(\pi, \barpzero^{\otimes n}) + 2\cRd.
\end{align*}
We now choose $\cRd \leq \frac{\eta}{2}$ and $\pi$ like in \eqref{prior_bulk} or in \eqref{prior_remainder} with $\barpzero$ instead of $p_0$, by imposing $d_{TV}(\pi, \barpzero^{\otimes n}) \leq 1-2\eta$, which can be done by choosing $\Cphi$ and $\cR$ small enough. This yields: $ d_{TV}(\widetilde{\Theta(\pi}), p_0^{\otimes n}) \leq 1-\eta$. Moreover, $\| \Theta(\pi)- p_0\|_t = \mathbb{P}_{p_0}(\Aout) \|\pi - \barpzero\|_t \geq \frac{1}{2}  \|\pi - \barpzero\|_t$. Hence we get:
$$ \rho_{\R^d}^*(p_0, \alpha, L, n) \gtrsim {\rhor}_{\Omega}(\barpzero, \alpha, L, n) + {\rhob}_{\Omega}(\barpzero, \alpha, L, n).$$
We now show that $\rho_{\R^d}^*(p_0, \alpha, L, n) \gtrsim {\rhot}_{\Omega}(\barpzero, \alpha, L, n)$ to complement this result. We let $\barqb$ be defined like in \eqref{def_prior_tail}, with $\barpzero$ instead of $p_0$. We take 
\begin{equation}\label{def_prior_tail_unbounded}
    p_b := \frac{\Theta(\barqb)}{\|\barqb\|_{1,\R^d}}.
\end{equation}
We have for fixed $b$:
\begin{align*}
    \big\|p_b - p_0\big\|_t &\geq \big\|p_b-p_0\big\|_{t,\Omega} \geq \big\|\barqb - \barpzero \big\|_{t,\Omega} -\big\|\barqb-p_b\big\|_{t,\Omega} -\big\|\barpzero-p_0\big\|_{t,\Omega}  \\
    & \geq \big\|\barqb - \barpzero \big\|_{t,\Omega}-  \big\|\barqb\big\|_{t,\Omega'}\Big|1-\frac{1}{\|\barqb\|_{1,\Omega'}}\Big| - \big\|p_0\big\|_{t,\Omega'}\Big|1-\frac{1}{\|p_0\|_{1,\Omega'}}\Big\|.
\end{align*}
Moreover, since $\barqb \in \mathcal{P}_1(\alpha,L',\cstar')$, it holds by Lemma \ref{control_norm_t_Rd}: $\|q_b\|_{t,\Omega} \leq \BL{\ref{control_norm_t_Rd}} {L'}^\frac{d(t-1)}{t(\alpha+d)}$, and $\|p_0\|_{t,\Omega} \leq \BL{\ref{control_norm_t_Rd}} {L'}^\frac{d(t-1)}{t(\alpha+d)}$. By Lemma \ref{norm_qb} we have with by Chebyshev's inequality that $\|q_b\|_{t,\Omega} \in [1 \pm \frac{4\sqrt{\CL{\ref{norm_qb}}}}{n\sqrt{\eta}}]$ with probability at least $1-\eta/4$. Therefore, with probability at least $1-\eta/4$:
\begin{align*}
    \big\|p_b - p_0\big\|_t & \geq \big\|\barqb - \barpzero \big\|_{t,\Omega}- 2\BL{\ref{control_norm_t_Rd}} \left(\frac{4\sqrt{\CL{\ref{norm_qb}}}}{\sqrt{\eta}} + 2\cRd\right)\rhor.
\end{align*}
\ju{Compléter pour la variation totale !!! De plus dans la dernière inégalité, gros problème car rien ne dit que c'est de l'ordre de $\rhot$ vu que la constante est grosse a priori.}\\

\underline{\textbf{Upper bound:}} ($\rho_{\R^d}^*(p_0, L,n) \lesssim \rho_{\Omega'}^*(\barpzero, L,n)$). 

Let $\barpsistar$ be an optimal test, i.e. such that $R_{\Omega'}(\barpsistar, \Cetoile \rho_{\Omega'}^*(\barpzero, L,n)) \leq \eta/4$ for $\Cetoile$ an absolute constant, sufficiently large. We define 
\begin{equation}\label{def_psi_out}
    \psiout := \mathbb{1}\left\{\bigvee\limits_{i=1}^n (X_i \notin \Omega')\right\},
\end{equation}
so that $\phi^* = \barpsistar \lor \psiout$. We show that there exists some absolute constant $C>0$ large enough, such that $R_{\R^d}(\psi^*, C\rho_{\Omega'}^*(\barpzero, L,n)) \leq \eta$, which proves that $\rho_{\R^d}^*(p_0, L,n) \leq C\rho_{\Omega'}^*(\barpzero, L,n)$, by definition.

\begin{itemize}
    \item Under $H_0$: Assume $X_1, \dots, X_n$ have density $p_0$ over $\R^d$. We have
    \begin{align*}
        \mathbb{P}_{p_0}\left(\psi^* = 1\right) &\leq \mathbb{P}_{p_0}\left(\barpsistar = 1\right) + \mathbb{P}_{p_0}\left(\psiout = 1\right) \leq \cRd + \eta/4 ~~ \text{ by union bound}\\
        & \leq \frac{\eta}{2}, ~~ \text{ by choosing $\cRd \leq \frac{\eta}{4}$.} 
    \end{align*}
    \item Under $H_1\left(C\rho_{\Omega'}^*(\barpzero, L,n)\right)$: Assume $X_1, \dots, X_n$ have density $p$ over $\R^d$, where $\|p-p_0\|_t \geq C\rho_{\Omega'}^*(\barpzero, L,n)$. We let $\cout$ be an absolute constant, sufficiently large. Assume first that $\int_{\R^d \setminus \Omega'} p > \frac{\cout}{n}$. Then:
    \begin{align*}
        \mathbb{P}_p\left(\psi^* = 0\right) &\leq \mathbb{P}_p\left(\psiout = 0\right)= \mathbb{P}_p\left(X_1 \in \Omega'\right)^n \leq \left(1-\frac{\cout}{n}\right)^n \leq e^{-\cout} \leq \frac{\eta}{2},
    \end{align*}
    for $\cout$ large enough. In this case, $R_{\R^d}(\psi^*, C\rho_{\Omega'}^*(\barpzero, L,n)) \leq \eta$. Now, and until the end of the proof, assume $\int_{\R^d \setminus \Omega'} p \leq \frac{\cout}{n}$. This yields by Lemma \ref{control_norm_t_Rd}:
        \begin{align*}
        \left\{\begin{array}{cc}
             \big\|p_0\big\|_{t,\Omega'} \leq \AL{\ref{control_norm_t_Rd}}(\cRd)\rhor\\
             \big\|p\big\|_{t,\Omega'} \leq \AL{\ref{control_norm_t_Rd}}(\cout)\rhor
        \end{array} \right. ~~ \text{ and } ~~ \left\{\begin{array}{cc}
             \Big|1-\frac{1}{\|p_0\|_{1,\Omega'}}\Big| \leq 2 \frac{\cRd}{n} \\
             \Big|1-\frac{1}{\|p\|_{1,\Omega'}}\Big| \leq 2 \frac{\cout}{n}
        \end{array}\right.
    \end{align*}
    Define:
    \begin{equation}\label{def_barp}
        \barp : \left\{\begin{array}{ccc}
             \Omega' &\longrightarrow &\R_+  \\
             x &\mapsto &p(x)/\int_{\Omega'} p
        \end{array}\right.
    \end{equation}
    Moreover, for any domain $\D \subset \R^d$ and any function $\phi: \R^d \longrightarrow \R$, denote by $\big\|p\big\|_{t,\D}$ the quantity $\left(\int_{\D}|\phi|^t\right)^{1/t}$. We have:
    \begin{align*}
        \big\|\barp - \barpzero\big\|_t &\geq \big\|p-p_0\big\|_{t,\Omega'} - \big\|p-\barp\big\|_{t, \Omega'} - \big\|p_0 - \barpzero\big\|_{t, \Omega'}\nonumber\\
        &= \big\|p-p_0\big\|_{t,\R^d} - \big\|p-p_0\big\|_{t,\R^d\setminus \Omega'} - \big\|p\big\|_{t,\Omega'}\Big|1-\frac{1}{\|p\|_{1,\Omega'}}\Big| ~ - ~ \big\|p_0\big\|_{t,\Omega'}\Big|1-\frac{1}{\|p_0\|_{1,\Omega'}}\Big|\\
        &\geq \big\|p-p_0\big\|_{t,\R^d} - (\AL{\ref{control_norm_t_Rd}}(\cout) + \AL{\ref{control_norm_t_Rd}}(\cRd))\rhor - 2\BL{\ref{control_norm_t_Rd}}\frac{\cout+ \cRd}{n}L^{\frac{d(t-1)}{t(\alpha+d)}}\\
        & \geq C\rho_{\Omega'}^*(\barpzero, L,n) - (\AL{\ref{control_norm_t_Rd}}(\cout) + \AL{\ref{control_norm_t_Rd}}(\cRd)-2\BL{\ref{control_norm_t_Rd}}(\cout+ \cRd))\rhor\\
        &\geq \Cetoile \rho_{\Omega'}^*(\barpzero, L,n),
    \end{align*}
    for $C$ large enough, since by definition: $\rhor \leq \rho_{\Omega'}^*(\barpzero, L,n) $. Therefore:
    \begin{align*}
    \mathbb{P}_p(\psi^*=0) = \mathbb{P}_p(\barpsistar=0 \cap \Aout) \leq \mathbb{P}_p(\barpsistar=0 | \Aout) \leq \frac{\eta}{4},
    \end{align*}
    by definition of $\barpsistar$.
\end{itemize}
\end{proof}

\begin{lemma}\label{control_norm_t_Rd}
Let $p \in \mathcal{P}_{\R^d}(\alpha,L,\cstar)$ and $\widetilde \Omega \subset \Omega$.
\begin{enumerate}
    \item If $\int_{\widetilde \Omega} p \leq \frac{c}{n}$ for some constant $c>0$, then 
    $$ \left(\int_{\widetilde  \Omega} p^t\right)^{1/t} \leq \AL{\ref{control_norm_t_Rd}}(c) \cdot \rhor,$$
    for $\AL{\ref{control_norm_t_Rd}}(c) $ an absolute constant depending only on $c, \eta, d, \alpha$ and $t$. Moreover, $\AL{\ref{control_norm_t_Rd}}(c) \underset{c \to 0}{\to} 0$ and $\AL{\ref{control_norm_t_Rd}}(c) \underset{c \to + \infty}{\to} + \infty$.
    \item There exists an absolute constant $\BL{\ref{control_norm_t_Rd}}$ such that $\|p\|_t \leq \BL{\ref{control_norm_t_Rd}} \cdot L^{\frac{d(t-1)}{t(\alpha+d)}}$.
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{control_norm_t_Rd}]
Let $x \in \R^d \setminus \Omega'$ and let $h = \left(\frac{p(x)}{4L}\right)^{1/\alpha}$. By Assumption \eqref{simplifyingAssumption}, we have for all $y \in B(x,h)$:
\begin{align*}
    p(y) \geq \frac{p_0(x)}{2} -L\left(\frac{p(x)}{4}\right) = \frac{p(x)}{4}.
\end{align*}
Moreover, since $\Omega'$ is a cube, $\text{Vol}\left(B(x,h) \cap (\R^d \setminus \Omega')\right) \geq \frac{1}{2}\text{Vol}(B(x,h))$. Therefore:
\begin{equation}\label{majorant_p_Rd}
    \int_{\R^d \setminus \Omega'} p ~\geq ~ \frac{p(x)}{4}\frac{1}{2}\text{Vol}(B(x,h)) ~ = ~ \Cd \frac{p(x)^{\frac{\alpha+d}{\alpha}}}{L^{d/\alpha}},
\end{equation}
where $\Cd = \frac{\text{Vol}\left(B(0,1)\right)}{8 \times 4^{d/\alpha}}$. 
\begin{enumerate}
    \item Therefore, if $\int_{\R^d \setminus \Omega'}p \leq \frac{c}{n}$, then $p(x) \leq \left(\frac{c}{\Cd}\frac{L^d}{n^\alpha}\right)^\frac{1}{\alpha+d}$, which yields:
\begin{align*}
    \int_{\R^d \setminus \Omega'} p^2 \leq \left(\frac{c}{\Cd}\frac{L^d}{n^\alpha}\right)^\frac{1}{\alpha+d} \times \frac{c}{n} = c \left(\frac{c}{\Cd}\right)^\frac{1}{\alpha+d}\frac{L^\frac{d}{\alpha+d}}{n^\frac{2\alpha + d}{\alpha + d}}.
\end{align*}
Now, by Hölder's inequality, we have
\begin{align*}
    \int_{\R^d \setminus \Omega'} p^t \leq \left(\int_{\R^d \setminus \Omega'} p\right)^{2-t}\left(\int_{\R^d \setminus \Omega'} p^2\right)^{t-1} =: \AL{\ref{control_norm_t_Rd}}^t(c) {\rhor}^t
\end{align*}
    \item The proof of the second assertion follows the same lines. We have by Equation \eqref{majorant_p_Rd} that $\forall x \in \R^d : 1=\int_{\R^d}p \geq \Cd \frac{p(x)^{\frac{\alpha+d}{\alpha}}}{L^{d/\alpha}}$, hence $p(x) \leq \frac{1}{\Cd^{\alpha/(\alpha+d)}}L^{\frac{d}{\alpha + d}}$ for all $x \in \R^d$. Therefore, $\int_{\R^d} p^2 \leq \frac{1}{\Cd^{\alpha/(\alpha+d)}}L^{\frac{d}{\alpha + d}} \int_{\R^d} p \leq \frac{1}{\Cd^{\alpha/(\alpha+d)}}L^{\frac{d}{\alpha + d}}$, so that by Hölder's inequality:
    \begin{align*}
    \int_{\R^d } p^t \leq \left(\int_{\R^d} p\right)^{2-t}\left(\int_{\R^d} p^2\right)^{t-1} = \Cd^{\frac{\alpha(1-t)}{\alpha+d}}L^{\frac{d(t-1)}{\alpha+d}} =: \BL{\ref{control_norm_t_Rd}}^t L^{\frac{d(t-1)}{\alpha+d}}.
\end{align*}
\end{enumerate}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ju{Brouillon :


We can now justify the assumptions $\min_\B \hB, \hT(\uA) < \homega$. 
\begin{itemize}
    \item Assume first that $\min_\B \hB < \homega$. If $\hT(\uA) > \homega$ then the condition $nL\homega^{\alpha+d} >\csmall$ and the definition of $\hT(\uA)$ yield $n\int_{\T(\uA)}p_0 < \frac{1}{\csmall} \leq \ctail$ for $\ctail$ large enough, hence $\rhot \leq \rhor$.
    \begin{itemize}
        \item The tail cannot dominate by Lemma \ref{htail_leq_hbulk}.
        \item Since the bulk dominates, Propositions \ref{upper_bound_bulk}, \ref{Lower_bound_bulk_proposition}, \ref{upper_bound_tail} and \ref{remainder_term} ensure that $\rho^* \asymp\rhob+\rhor$.
    \end{itemize}
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{lemma}\label{very_small_p_0}
Suppose that the tail dominates, \textit{i.e.} $\rhot \geq \CBT \rhob$ %\al{$\CBT$ est il defini? Et $\cA$?}
and set $v := \frac{4}{\cA}\uA$. Then for all $j \geq U$, if $\exists z \in \widetilde C_j$ such that $p_0(z) \geq v$ then $p_j \geq \frac{vh^d}{4}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{very_small_p_0}]
Suppose that for some $j \geq U$ and some $z \in \widetilde C_j$ we have $p_0(z) \geq v$. Then by Assumption \eqref{simplifyingAssumption}:
\begin{align*}
    \int_{\widetilde C_j} p_0 &\geq \int_{\widetilde C_j} (1-\cstar)v - L \|x-z\|^\alpha dx \geq (1-\cstar) v h^d -  L h^{\alpha + d}\\
    & \geq \frac{v h^d}{2} -  L h^d \inf_\B \hB^\alpha =  h^d \left[\frac{v}{2} -  \frac{1}{\cA} \uA \right] = \frac{v}{4} h^d.
\end{align*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{sum_pj_geq_int}
Suppose the tail dominates, i.e.: $\rhot \geq \CBT \rhob$. There exists an absolute constant $D$ % $D = \frac{\cu}{6\Cstep}$ \ju{A modifier}
such that whenever $\int_{\T(\uA)} p_0 \geq \frac{\ctail}{n}$, it holds: $$\sum_{j\geq U} p_j \geq D \int_{\T(\uA)} p_0.$$ Moreover, $D$ \ssmall{$\cu$} and $\ctail$ large enough.
%When $\int_{\T(\uA)}p_0 \geq \frac{\ctail}{n}$ and $\rhot \geq \CBT \rhob$, it holds:
%$$ \sum_{j\geq U} p_j \geq \Big(D \land \frac{1}{2} \Big) \int_{\T(\uA)} p_0.$$
%\ju{Ajuster $\Cmom$ pour que $D \leq \frac{1}{2}$ }
\end{lemma}

%\ju{Changer $D$ en $\CL{\ref{sum_pj_geq_int}}$ partout ?}

\begin{proof}[Proof of Lemma \ref{sum_pj_geq_int}]
\hfill

\begin{itemize}
    \item \underline{\textbf{First case:}} $p_U \leq  \Cstep Lh^{\alpha+d}$. If $U=1$ then since $\T(\uA) \subset \bigcup\limits_{j=1}^M \widetilde C_j$, we have $\sum\limits_{j\geq U} p_j \geq \int_{\T(\uA)} p_0$ hence the result is clear. Assume now that $U \geq 2$ and that $p_U \leq \Cstep L h^{\alpha + d}$. We can then write, by definition of $U$:
\begin{align*}
    p_{U-1} \sum_{j \geq U-1} p_j > \frac{\cu}{n^2},
\end{align*} where $p_{U-1} \leq \Cstep' L h^{\alpha+d}$ by Lemma \ref{only_small_jumps}. Therefore:
\begin{align*}
    \sum_{j \geq U} p_j &> \frac{\cu}{n^2 p_{U-1}} - p_{U-1} \geq \frac{\cu}{n^2 \Cstep' L h^{\alpha + d}} - \Cstep' L h^{\alpha + d}\\
    & = \frac{\cu}{\Cstep'} \int_{\T(\uA)} p_0 - \frac{\Cstep'}{n^2 \int_{\T(\uA)} p_0}\\
    & \geq \frac{\cu}{\Cstep'} \int_{\T(\uA)} p_0 - \frac{\Cstep'}{\ctail^2} \int_{\T(\uA)} p_0\geq D \int_{\T(\uA)} p_0.
\end{align*}
Choosing $\ctail^2 \geq \frac{\Cstep'^2}{2\cu}$ yields the result with $D = \frac{\cu}{\Cstep'} - \frac{\Cstep'}{\ctail^2}$. %then by Lemma \ref{pU_small_sum_large}, the result holds.
    \item \underline{\textbf{Second case:}} $p_U > \Cstep Lh^{\alpha+d}$. Since by Lemma \ref{very_small_dominate} we have $\T(2\Cmom L h^\alpha) \neq \emptyset $, let $j \in \Ibar$ such that $\widetilde C_j \cap \T(2\Cmom L h^\alpha) \neq \emptyset$. Let $y_j \in \widetilde C_j \cap \T(2\Cmom L h^\alpha)$. We have by Assumption \eqref{simplifyingAssumption} for all $x \in \widetilde C_j$: $p_0(x) \leq (1+\cstar) p_0(y_j) + L(h \sqrt{d})^\alpha$ so that: $p_j \leq (1+\cstar)p_0(y_j) h^d + Lh^{\alpha + d} \sqrt{d}^\alpha \leq \left( (1+\cstar)2\Cmom + \sqrt{d}^\alpha \right)L h^{\alpha + d} \leq \Cstep Lh^{\alpha + d} < p_U$ by choosing $\Cmom$ small enough (which can be done by choosing successively $\cA$ and $\cI$ small enough) so that $j >U$. Moreover, since by assumption we have $\rhot \geq \CBT \rhob$, we have by Lemma \ref{htail_leq_hbulk}: $2\Cmom Lh^\alpha \leq \frac{2\Cmom}{\CBT^{(2)}}  L \inf_{\B}\hB^\alpha \leq \cA L \inf_{\B}\hB^\alpha \leq \uA$ by choosing $\CBT^{(2)}$ small enough, which can be done by choosing $\CBT$ small enough. Therefore: $\T(2\Cmom Lh^\alpha) \subset \T(\uA)$, which yields: 
    \begin{align*}
        \sum_{j \geq U} p_j \geq \int_{\T(2\Cmom L h^\alpha)} p_0 \geq \frac{1}{2} \int_{\T(\uA)} p_0 ~~ \text{ by Lemma \ref{very_small_dominate}.} 
    \end{align*}
\end{itemize}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{Toute_la_case_OK_moment1}
In the case where the tail dominates, \textit{i.e.} when $\rhot \geq \CBT \rhob$, there exists an absolute constant $\CL{\ref{Toute_la_case_OK_moment1}}$ such that $\sum\limits_{j \geq U} p_j \leq \CL{\ref{Toute_la_case_OK_moment1}} \int_{\T(\uA)} p_0$. %\ju{A raffiner pour avoir $\CBT$ proportionnel à $\cu$.}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Toute_la_case_OK_moment1}]
Set $h = \hT(\uA)$.
\begin{itemize}
    \item \underline{\textbf{First case:}} Assume that $p_U \leq L h^{\alpha+d}$. Then by Assumption \eqref{simplifyingAssumption}, it holds
    \begin{align*}
        \max\limits_{\widetilde C_j} p_0 \leq (1+\cstar) Lh^\alpha + L(h\sqrt{d})^\alpha \leq (1+\cstar + \sqrt{d}^\alpha) \frac{1}{{\CBT^{(2)}}^\alpha} \frac{1}{\cA} \uA \leq \frac{\uA}{2}
    \end{align*}
    by choosing $\CBT^{(2)}$ large enough, which can be done by choosing $\CBT$ large enough. It follows that $\bigcup\limits_{j\geq U} \widetilde C_j \subset \T(\uA)$ hence $\sum\limits_{j\geq U} p_j \leq \int_{\T(\uA)}p_0$.
    \item \underline{\textbf{Second case:}} $p_U > L h^{\alpha+d}$. Then:
    \begin{align*}
        \sum_{j\geq U}p_j \leq \frac{\cu}{n^2p_U} < \frac{\cu}{n^2L h^{\alpha+d}} = \cu \int_{\T(\uA)}p_0.
    \end{align*}
\end{itemize}



\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{Toute_la_case_OK_moment2}
Whenever the tail dominates, \textit{i.e.} when $\rhot \geq \CBT \rhob$, there exists an absolute constant $\CL{\ref{Toute_la_case_OK_moment2}}$ such that $\int_{\bigcup\limits_{j \geq U} \widetilde C_j} p_0^2 \leq \CL{\ref{Toute_la_case_OK_moment2}} \, \frac{1}{n^2 h^d}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Toute_la_case_OK_moment2}]

and let $J_{\text{large}} = \{j \geq U: \sup_{\widetilde C_j} p_0 \geq \uA\}$.


\begin{itemize}
    \item We have by definition of $\T(\uA)$ that $\bigcup_{j \notin J_{\text{large}}} \widetilde C_j \subset \T(\uA)$, which yields by Lemma \ref{int_p0squared_uA_small}: \\ $\int_{\bigcup_{j \notin J_{\text{large}}} \widetilde C_j} p_0^2 \leq \frac{\Cmom}{n^2 h^d}$.
    \item For all $j \in J_{\text{large}}$, let $y_j \in \widetilde C_j$ such that $p_0(y_j) > \uA$ and $z_j \in \widetilde C_j$ such that $p_0(z_j) < \uA$. By Assumption \eqref{simplifyingAssumption} we have for all $x \in \widetilde C_j: p_0(x) \geq (1-\cstar) p_0(y_j) - L h^\alpha \sqrt{d}^\alpha \geq \frac{1}{2}\cA L \inf_{\B}\hB^\alpha - Lh^\alpha \sqrt{d}^\alpha \geq \frac{\uA}{4} h^\alpha$, so that $p_j \geq \frac{\uA}{4} h^{\alpha + d}$. Moreover, $p_0(x) \leq (1+\cstar)p_0(y_j) + Lh^\alpha \sqrt{d}^\alpha$. Therefore:
    \begin{align*}
        \int_{\widetilde C_j} p_0^2 &\leq p_j\left[(1+\cstar)p_0(z_j) + Lh^\alpha \sqrt{d}^\alpha\right] \leq \left[1 + \cstar + \frac{\sqrt{d}^\alpha}{\cA} \right] \uA p_j \leq 4 \left[1 + \cstar + \frac{\sqrt{d}^\alpha}{\cA} \right] p_j^2 h^{-d},
    \end{align*}
    hence:
    \begin{align*}
        \int_{\hspace{-3mm} \bigcup\limits_{j \in J_{\text{large}}} \hspace{-3mm} \widetilde C_j} p_0^2 ~~ &\leq 4 \left[1 + \cstar + \frac{\sqrt{d}^\alpha}{\cA} \right] \sum_{j \geq U} p_j^2 h^{-d} \leq \frac{4 \left[1 + \cstar + \frac{\sqrt{d}^\alpha}{\cA} \right] \cu}{n^2 h^d}.
    \end{align*}
\end{itemize}
Hence, setting $\CL{\ref{Toute_la_case_OK_moment2}} = \Cmom +  4 \left[1 + \cstar + \frac{\sqrt{d}^\alpha}{\cA} \right]  \cu$, we get the result.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}\label{perturbation}
     \phi_j(x) = \Cphi L \Big(h_j - \big\|x-x_j - \frac{h_j}{\sqrt{d}}\overset{\rightarrow}{\mathbb{1}} \big\| \Big)_+^\alpha -  \Cphi L \Big(h_j - \big\|x-x_j + \frac{h_j}{\sqrt{d}}\overset{\rightarrow}{\mathbb{1}} \big\| \Big)_+^\alpha,
\end{equation}\al{Est ce vraiment $\alpha$-Holder, ou faut il faire qqchose ici? (cf partie positive plus m!)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{gammaup_simplifying_assumption}
For some $h>0$ and $c'>0$ let $\gamma(x) = \lambda L(h-\|x\|)_+^\alpha$ where $\lambda \leq c'/c''$ and $c'' = \max \left\{\frac{1-(1+\cstar)(1-a)^\alpha}{a^\alpha} : a \in \left[0, 1\right]\right\}$. Then $\forall (x,y) \in \R^d, |\gamma(x) - \gamma(y)| \leq \cstar \gamma(y) + c' L \|x-y\|^\alpha$. 
\end{lemma}

\begin{proof}[Proof of Lemma \ref{gammaup_simplifying_assumption}]
The real number $c''$ is well-defined, since for $a \leq 1-(1+\cstar)^{-1/\alpha}$, the quantity $\frac{1-(1+\cstar)(1-a)^\alpha}{a^\alpha}$ is negative, whereas the function $a \mapsto \frac{1-(1+\cstar)(1-a)^\alpha}{a^\alpha}$ is positive and continuous on the compact set $\left[1-(1+\cstar)^{-1/\alpha},1\right]$. Let $x,y\in \R^d$ and suppose by symmetry $\gamma(x) \geq \gamma(y)$. Set $u = \min\{u\geq 1: \gamma(ux) = \gamma(y) \}$. The real number $u$ is well-defined and satisfies $u \leq \frac{1}{x_0}$. Since $\{y' \in \R^d : \gamma(y') = \gamma(y)\}$ is a sphere, we have $\|x-ux\| \leq \|x-y\|$. We now show $\gamma(x) - \gamma(ux) \leq \cstar \gamma(ux) + c'L\|x-ux\|^\alpha$, which will prove the result. \\

If $\|x\| \geq h$ then the result is clear. Otherwise, set $x_0 = \left\|\frac{x}{h}\right\|$ and % and $u_0 = c' \left(1 \land \frac{(1- v)^\alpha}{1-v^\alpha}\right)$ where $v = (1+\cstar)^{-\frac{1}{\alpha}}$. We have $\phi(x) = Lh^\alpha(1-x_0)_+^\alpha$ and $\phi(ux) = Lh^\alpha(1-ux_0)_+^\alpha$. 
$a = \frac{u-1}{\frac{1}{x_0}-1} \in [0,1]$ (since $u \leq 1/x_0$). We therefore have:
\begin{align*}
\gamma(x) - (1+\cstar) \gamma(ux) - c'L\|x-ux\|^\alpha = \left(1-x_0\right)^\alpha\left[c\big(1-(1+\cstar)(1-a)^\alpha\big) - c'a^\alpha\right] \leq 0,
\end{align*}
which ends the proof.
\end{proof}

\begin{lemma}\label{gammaup_simplifying_assumption_cases_diff}
Let $I$ be a countable set of indices and $(x_l)_{l \in I} \in \Omega$ and $(h_l)_{l \in I} >0$ such that the balls $(B(x_l, h_l))_l$ are disjoint. Set moreover $(\epsilon_l)_{l \in I} \in \{\pm 1\}^I$. Let $\lambda, c'>0$ be defined like in Lemma \ref{gammaup_simplifying_assumption}. Let $\Calpha =1 \lor 2^{1-\alpha}$ and $\gamma(x) = \lambda\sum_{l=1}^j \epsilon_l L(h_l - \|x-x_l\|)_+^\alpha$. Then $\forall x,y \in \Omega, |\gamma(x) - \gamma(y)| \leq \cstar |\gamma(x)| + c' \Calpha L \|x-y\|^\alpha$.
\end{lemma}


\begin{proof}[Proof of Lemma \ref{gammaup_simplifying_assumption_cases_diff}]
Set for all $l \in I: A_l = B(x_l, h_l)$ and $A_{0} = \Omega \setminus \left(\bigcup_{l \in I} A_l \right)$. Let $x,y \in \Omega$. If $x,y$ are in the same set $A_l$ then the result follows from Lemma \ref{gammaup_simplifying_assumption} (or is direct if $x,y \in A_{0}$). Assume there exist $i \neq l$ such that $x \in A_i$ and $y \in A_l$. For $x'\in A_i$ and $y' \in A_l$ such that $d_{\|\cdot\|}(x',A_{0}) =0$ and $d_{\|\cdot\|}(y',A_{0}) =0$ we have by Lemma \ref{gammaup_simplifying_assumption}: $$|\gamma(x)| = |\gamma(x)| - |\gamma(x')| \leq \cstar |\gamma(x')| + c'L\|x-x'\|^\alpha = c'L\|x-x'\|^\alpha,$$ $$|\gamma(y)| = |\gamma(y)| - |\gamma(y')| \leq \cstar |\gamma(y')| + c'L\|y-y'\|^\alpha = c'L\|y-y'\|^\alpha.$$ 

\hfill

Moreover, we have $\|x-y\| \geq \|x-x'\| + \|y-y'\|$ since $x$ and $y$ are in two different sets, and $\Calpha = \max \{\lambda^\alpha + (1-\lambda)^\alpha: \lambda \in [0,1]\}$ so that: $\Calpha\|x-y\|^\alpha \geq \|x-x'\|^\alpha + \|y-y'\|^\alpha$. This yields the result.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    
    
    To finish we show that Assumption \eqref{simplifyingAssumption} is satisfied with the constants $(1+\cdown)L$ and $(1+\cdown)\cstar$ instead of $L$ and $\cstar$. We have
    $$ \philj(x) \leq \cdown L\big(\hlj\big)^\alpha = \cdown L\Big[\Big(\frac{p_0(\zlj)}{\cbeta}\Big)^{1/\alpha}\Big]^\alpha \leq \cdown \cdot 2^\alpha \frac{p_0(x)}{\cbeta'},$$
    recalling that $\cbeta'$ is an absolute constant which can be chosen large enough to ensure the assumptions of Lemma \ref{gammaup_simplifying_assumption_cases_diff}. It follows that for all $x,y \in \Omega$:
    \begin{align*}
        &\left|\left(p_0 - \gammadown\right)(x)-\left(p_0 - \gammadown\right)(y)\right| \leq \left|p_0(x)-p_0(y)\right| + \left|\gammadown(x)-\gammadown(y)\right|\\
        & \leq \left|p_0(x)-p_0(y)\right| + |\gamma(x) - \gamma(y)| \leq \left|p_0(x)-p_0(y)\right| + \cstar |\gammadown(x)| + c' \Calpha L \|x-y\|^\alpha\\
        & \leq \cstar\left(p_0(x) + \gammadown(x)\right) + (1+c' \Calpha)L\|x-y\|^\alpha\\
        & \leq \cstar\frac{1+\frac{\cdown}{\calpha}}{1-\frac{\cdown}{\calpha}}\left(p_0(x) - \gammadown(x)\right) + (1+c' \Calpha)L\|x-y\|^\alpha\\
        & \leq \cstar'\left(p_0(x) - \gammadown(x)\right) + L'\|x-y\|^\alpha , ~~ \text{  by choosing $\cdown$ and $c'$ small enough.}
    \end{align*}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Lemma \ref{Toute_la_case_OK_moment1}]
Set $h = \hT(\uA)$.
By Assumption \eqref{simplifyingAssumption}, Lemma \ref{pU_leq_Lh^alpha+d} and Lemma \ref{htail_leq_hbulk}, it holds
    \begin{align*}
        \max\limits_{\widetilde C_j} p_0 \leq (1+\cstar) \CL{\ref{pU_leq_Lh^alpha+d}} Lh^\alpha + L(h\sqrt{d})^\alpha \leq \left((1+\cstar) \CL{\ref{pU_leq_Lh^alpha+d}} + \sqrt{d}^\alpha \right) \frac{1}{{\CBT^{(2)}}^\alpha} \frac{1}{\cA} \uA \leq \frac{\uA}{2}
    \end{align*}
    by choosing $\CBT^{(2)}$ large enough, which can be done by choosing $\CBT$ large enough. It follows that $\bigcup\limits_{j\geq U} \widetilde C_j \subset \T(\uA)$ hence $\sum\limits_{j\geq U} p_j \leq \int_{\T(\uA)}p_0$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\ju{Questions:
%\begin{itemize}
    %\item Est-ce que le terme résiduel $\frac{1}{n}$ apparaît dans le rate ? On dirait qu'on en a besoin dans la preuve de la borne sup pour le tail dans le test $\psi_1$. 
    %\item Est-ce qu'on pourrait écrire la preuve pour un domaine non borné ?
    %\item Est-ce qu'on peut faire un poissonization trick pour généraliser aux processus de poisson spatiaux plutôt que de rester en densités ?
    %\item Quelle réf on a pour dire que $|p(x) - \hat{p}(x)| \leq L h(x)^\alpha$ quand on a un noyau d'ordre $\alpha$ en dim $d$ ? Dans le livre de Sacha il n'y a que la dimension 1.
    %\item Quand on fait le partitionnement Bulk-Tail par rapport à $\uA$ puis qu'on fait le splitting en cubes il n'y a pas de raison que chaque cube soit inclus dasn soit Bulk soit tail (un cube peut être à cheval sur Bulk et Tail).
    %\item Comment on fait le prior sparse pour qu'il soit bien dans $H(\alpha, L)$ ? De plus comment on fait pour qu'il soit bien d'intégrale $0$ ?
    %\item Pour la borne sup bulk : on arrive à montrer que le rate est le bon pour $n$ suffisamment grand. En particulier on montre sous $H_1$ que $\V(\Tb) \lesssim \E(\Tb)^2\frac{C}{n^2} $ pour une grosse constante $C$. Cependant, pourquoi cela donne le bon rate de dire que "pour $n$ assez grand" on a $C/n^2 \ll 1$ ? En effet quand on prend $n=1$ dans le rate, le terme résiduel est plutôt en $L^{\frac{d(1-1/t)}{\alpha+d}}/n^{\frac{\alpha t + d}{\alpha + d}}$
    %\item J'arrive à peu près à faire le recollement pour le prior tail mais je n'arrive pas à montrer qu'il est $\alpha$-Hölder. 
    %\item Je n'arrive pas à montrer que la variation totale entre le prior et $p_0^{\otimes n}$ est petite.
    %\item Je n'arrive pas à faire le poissonization trick.
    %\item Pour toutes les intégrales $\int_{\overline \T(u)} p_0^2$, qu'est-ce qu'il se passe si $u > \max p_0$ ?
    %\item Il se passe quoi si $\hB \geq 1$ ou $Ln \geq 1$ ?
    %\item Nos résultats sont vrais pour $n$ assez grand mais juste plus grand qu'une constante absolue indépendante de $p_0$, est-ce que c'est asymptotique ou pas ?
%\end{itemize}
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Arbitrary $p_0$ over $\Omega = [0,1]^d$ with $L=1$}

By Ascoli's theorem, $\left(\mathcal{P}(\alpha,L,\cstar), \|\cdot\|_{\infty}\right)$ is compact. Moreover, $p \mapsto \rho^*(p)$ is continuous over $\mathcal{P}(\alpha,L,\cstar)$. Indeed, we first note that for all $p,q \in \mathcal{P}(\alpha,L,\cstar)$ we have $d_{TV}(p^{\otimes n}, q^{\otimes n}) \leq n\|p-q\|_{\infty}$ and $\|p - q\|_t \leq \|p-q\|_\infty$ over $\mathcal{P}(\alpha,L,\cstar)$ since all functions are defined over $[0,1]^d$. Let $q_0 \in \mathcal{P}(\alpha,L,\cstar)$. For all $\epsilon > 0$, there exists a test $\psi$ such that $\forall p \in \mathcal{P}(\alpha,L,\cstar)$, $\|p-q_0\|_t > \rho^*(q_0, \eta-\epsilon) \Longrightarrow \mathbb{P}_p(\psi=0) + \mathbb{P}_{q_0}(\psi=1) \leq \eta-\epsilon$. Now let $p_0 \in \mathcal{P}(\alpha,L,\cstar)$ such that $\|p_0-q_0\|_\infty \leq \frac{\epsilon}{n}$, so that $d_{TV}(p^{\otimes n}, q^{\otimes n}) \leq \epsilon$. We have for the same test: 
\begin{align*}
    \mathbb{P}_p(\psi=0) + \mathbb{P}_{p_0}(\psi=1) \leq \mathbb{P}_p(\psi=0) + \mathbb{P}_{q_0}(\psi=1) + d_{TV}(p_0^{\otimes n}, q_0^{\otimes n}) \leq \eta,
\end{align*}
hence $\rho^*(p_0, \eta)\leq \rho^*(q_0,\eta-\epsilon) + \|p_0-q_0\|_t$. Now, letting $\epsilon \to 0$ we get $\lim\sup\limits_{p_0 \to q_0}\rho^*(p_0, \eta)\leq \rho^*(q_0,\eta)$. By the same steps, we can also write, for fixed $q_0$: $\rho^*(q_0,\eta+\epsilon)\leq \rho^*(p_0,\eta)+\|p_0-q_0\|_t$ whenever $\|p_0-q_0\|_\infty\leq \frac{\epsilon}{n}$. Hence $\lim\inf\limits_{p_0 \to q_0}\rho^*(p_0, \eta) \geq \rho^*(q_0, \eta+\epsilon)$ for all $\epsilon$, hence $\lim\inf\limits_{p_0 \to q_0}\rho^*(p_0, \eta) \geq \rho^*(q_0, \eta)$ and $\rho^*$ is continuous. This fact being established, and noting that $\rho^*>0$ over $\mathcal{P}(\alpha,L,\cstar)$, the function
$$ \left\{ \begin{array}{ccc}
     \mathcal{P}(\alpha,L,\cstar)& \longrightarrow & \R_+^*  \\
     p_0 & \longmapsto & \rho^*(p_0)/\rho^*(1) 
\end{array}\right.$$
is continuous over a compact set and never reaches $0$ (we here denote by $1$ the density of the uniform distribution over $[0,1]^d$). Therefore, there exist two absolute constants $c,C$ such that for all $p \in \mathcal{P}(\alpha,L,\cstar): c \rho^*(1) \leq \rho^*(p_0) \leq C \rho^*(1)$.

\ju{on a utilisé que $\eta \longmapsto \rho^*(p_0,\eta)$ est continue, pourquoi c'est évident ?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Partitioning scheme}

We now focus on the procedure splitting each of the parts - bulk and tail - into smaller cubes with suitable edge lengths. On the bulk, the optimal splitting $(B_j)_j$ involves cubes of different edge lengths $(\cch\hB(x_j))_j$ where $\cch$ is a small absolute constant. On the tail, the optimal splitting consists of cubes of the same edge length $\asymp \hT$. These edge lengths are defined as follows:
\begin{itemize}
    \item For each $x \in \B(\frac{\uA}{2})$, the optimal edge length depends on the value $p_0(x)$ as:
    \begin{equation}\label{def_hbulk}
        \hB(x) = \frac{p_0(x)^\frac{2}{(4-t)\alpha + d}}{\Big(n^2 L^4 \, \I \Big)^\frac{1}{4\alpha + d}}.
    \end{equation}
    Note that $\hB$ is defined on $\B(\frac{\uA}{2})$ instead of $\B = \B(\uA)$, which will play a role in the analysis of the bulk regime. %\ju{On a peut-être même besoin de $\hB$ défini sur le bulk} \al{?}
    \item Recalling that $\T = \T(\uA)$, we moreover define:
    \begin{equation}\label{def_htail}
        \hT := \Big(n^2 L\; p_0[\T]\Big)^{-\frac{1}{\alpha + d}}.
    \end{equation}
\end{itemize}
%\ju{Est-ce qu'on a besoin de $1 \land \dots$ ?}
%\ju{J'ai l'impression de ne jamais utiliser $\hT(\uI)$ mais seulement $\hT(\uA)$. D'autre part est-ce que si $\hT=1$ alors le tail ou le bulk domine ?} \al{A garder en tete pour la finalisation de tout ca: soit ca passe, soit on exclue le cas par uen hypothese.}\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Ancienne preuve Lemme  Erreur_II_psi2

\begin{proof}
We draw $\widetilde k \sim \Poi(k)$ where we recall that $k = \frac{n}{2}$. We consider the setting where we observe $\widetilde X_1, \dots, \widetilde X_{\widetilde k}$ iid drawn from the density $p$ and define $\forall j \in \Ibar, N_j' = \sum_{i=1}^{\widetilde k} \mathbb{1}_{\widetilde X_i = j}$ the histogram of the tail in this modified setting. We recall that by the classical poissonization trick, the random variables $(N'_j)_j$ are independent and distributed as $\Poi(kq_j)$ respectively. We first notice that
\begin{align}
    \mathbb{P}_{p^{\otimes \widetilde k}}(\forall j \in \Ibar: N_j' = 0 \text{ or } 1) &\geq \mathbb{P}_{p^{\otimes \widetilde k}}(\forall j \in \Ibar: N_j' = 0 \text{ or } 1| \widetilde k \leq n)\mathbb{P}(\widetilde k \leq n)\nonumber \\
    & \geq \mathbb{P}_{p^{\otimes n}}(\forall j \in \Ibar: N_j' = 0 \text{ or } 1)\mathbb{P}(\widetilde k \leq n)\label{histogram_poissonized}
\end{align}
Moreover, 
\begin{align*}
    &\mathbb{P}_{p^{\otimes \widetilde k}}(\forall j\in \Ibar : N_j = 0 \text{ or } N_j = 1)  \; = \prod_{j \in \Ibar} \left[(1-q_j)^k + kq_j(1-q_j)^{k-1}\right]\\
     = &\prod_{j \in \Ibar}(1-q_j)^{k-1}(1+(k-1)q_j) \; = \; \prod_{j \in \Ibar}(1-q_j)^{k'}(1+k'q_j), \text{ writing } k'=k-1
\end{align*}
    Let $I_{-} = \{j\in \Ibar: kq_j \leq \frac{1}{2}\}$ and $I_{+} = \{j\in \Ibar: kq_j > \frac{1}{2} \}$. Recall that for $x\in (0,1/2], \; \log(1+x) \leq x - x^2/3$. Then, for $j \in I_-$: 
    \begin{align*}
        (1-q_j)^{k'}(1+k'q_j) &= \exp\left\{k' \log(1-q_j) +\log(1+k'q_j)\right\}\\
        & \leq \exp\left\{-k' q_j +k'q_j - \frac{k'^{\; 2}q_j^2}{3} \right\}\\
        & = \exp\left(- \frac{k'^{\; 2}q_j^2}{3}\right)
    \end{align*}
    
    Now, for $j \in I_+$, we have: $  k'\log(1-q_j) + \log(1+k'q_j) \leq -k'q_j + \log(1+k'q_j) \leq -\frac{1}{10} k'q_j
$ using the inequality $-0.9x + \log(1+x) \leq 0$ true for all $x \geq \frac{1}{2}$. 
Therefore, we have upper bounded the type-II error of $\psi_2$ by:
\begin{align*}
    \mathbb{P}_{p^{\otimes \widetilde k}}(\forall j\in& \Ibar : N_j = 0 \text{ or } N_j = 1) \leq \exp\Big(-\frac{1}{3} \sum_{j \in I_-} k'^{\; 2}q_j^2 - \frac{1}{10} \sum_{j\in I_+} k'q_j\Big)\\
    & \leq \exp\Big(-\frac{1}{3} \sum_{j \in I_-} k'^{\; 2}q_j^2 - \frac{1}{10}\big(\sum_{j\in I_+} k'^{\; 2}q_j^2\big)^{1/2}\Big)\\
    & = \exp\Big(-\frac{1}{3} (S-S_+) - \frac{1}{10}\left(S_+\right)^{1/2}\Big) \text{ for $S = \sum_{j\in \Ibar} k'^{\; 2}q_j^2$ and $S_+ = \sum_{j\in I_+} k'^{\; 2}q_j^2$.} 
\end{align*}
Now, $S_+ \mapsto -\frac{S}{3} + \frac{1}{3}S_+ - \frac{\sqrt{S_+}}{10}$ is convex over $[0,S]$ so its maximum is reached on the boundaries of the domain and is therefore equal to $(-\frac{\sqrt{S}}{10}) \vee -\frac{S}{3} = -\frac{\sqrt{S}}{3}$ for $S \geq 9/100$. Now, since $\|q\|_2^2 \geq 4\CL{\ref{Erreur_II_psi2}}/k^2 \geq \CL{\ref{Erreur_II_psi2}}/k'^{\; 2}$, we have $S = k'^{\; 2} \|q\|_2^2 \geq \log(16/\eta)^2 \vee 9/100$ which ensures $\mathbb{P}_{p^{\otimes \widetilde k}}(\forall j\in \Ibar : N_j = 0 \text{ or } N_j = 1) \leq \eta/16$, hence, by equation \eqref{histogram_poissonized}, $\mathbb{P}_p(\psi_2 = 0) \leq \frac{\eta}{16}/\mathbb{P}(\widetilde k \leq n) \leq \frac{\eta}{8}$ if $n$ is larger than a constant.% \ju{Vérifier pour les constantes et choisir $n$ assez grand pour que $\mathbb{P}(\widetilde k \leq n) \geq \frac{1}{2}$.}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

More precisely, on each cube $B_j$, we define an undetectable perturbation in a sense specified below. 
We first define a \textit{bounded} cubic domain $\widetilde \Omega \subset \Omega$ containing $\B$\boundedcase{ (if $\Omega$ is already bounded, we directly take $\widetilde \Omega = \Omega$)}. 
We apply Algorithm \ref{Algo_partitionnement} from Appendix \ref{Algo_appendix} with inputs given in Appendix \ref{Lower_bound_bulk_appendix}, which yields a covering of the bulk denoted throughout as $(B_1, \dots, B_N)$, for some $N \in \N$. 
The cells $B_j$ do not intersect and by construction $\B \subset \cup_{j} B_j$, while the reverse inclusion may not necessarily hold. 
Note that our prior is supported on $\cup_{j} B_j$ rather than on $\B$, which will nonetheless yield the desired rate provided that the bulk dominates.\\

%%%%%%%%%%%%%%%%%%%%%%%%%

On each cell $B_j$, we add to $p_0$ a random perturbation $\epsilon_j \phi_j$ where $(\epsilon_j)_j$ are iid centered Rademacher random variables and where $\phi_j \in H(\alpha, \delta L)$ is deterministic and supported on $B_j$. 
Each perturbation $\phi_j$ is chosen so that $\int_{B_j} \phi_j = 0$ and $p_0\pm \phi \geq 0$ over $B_j$. 


%%%%%%%%%%%%%%%%%%%%%%%

The magnitude of $(\phi_j)_j$ and the edge lengths of $(B_j)_j$ are optimized so as to maximize the $L_t$ discrepancy $\|p_\epsilon^{(n)}-p_0\|_t = \|\sum_j \phi_j\|_t$, subject to $d_{TV}\big(p_\epsilon^{(n)}, p_0^{\otimes n}\big) \leq 1-\eta$. 
Moreover, the cut-off $\uA$ can be understood as the smallest value (up to multiplicative constant) ensuring the condition $p_0 \pm \phi_j \geq 0$ over $\B(\frac{\uA}{2})$ once the $(\phi_j)$ have been optimally chosen. 




%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Cut-offs}

%The value $\uI$ is an auxiliary value defined so that, after splitting $\T(\uI)$ into cubes with edge length $\hT(\uI)$, no same cell contains two observations or more \textit{whp}. 
A nice property of $\uA$ (see Lemma \ref{proba_observed_twice}) is that if the tail dominates, then after splitting $\T(\uA)$ into cubes with edge length $\hT$, any tail cube should contain either zero or one observation \textit{whp} under $H_0$. 
Unfortunately, this condition no longer holds if the bulk dominates, which is the reason why we split $\T(\uA/2)$ into cubes of edge length $\asymp \hm \leq \min\limits_{\B(\uA)}\hB$ in this case. % - so that the data structure over the cubes in $\T(\uA)$ is quite simple. 
Here is some intuition on why in some cases we consider $\B(\frac{\uA}{2})$ or $\T(\frac{\uA}{2})$ instead of $\B(\uA)$ and $\T(\uA)$.
Indeed, it is not always possible to set the optimal bulk prior \eqref{prior_bulk} over $\B(\uI)$. 
This leads us to introduce the smallest cut-off $\uA\geq \uI$ ensuring that \eqref{prior_bulk} can be supported on $\B(\uA)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another way of justifying Assumption~\eqref{simplifyingAssumption}'s mildness is as follows. 
If a density $p$ violates Assumption~\eqref{simplifyingAssumption}, then it satisfies $|p(x)-p(y)|\gg \cstar p(x) + L\|x-y\|^\alpha$ for some $x,y\in\R^d$. 
%By symmetry, assume that $p(y)> p(x)$. 
On some parts of the line from $x$ to $y$, the function $p$ therefore needs to increase very fast. 
However, by the Hölder condition, $p$ necessarily remains increasing on a large part of the domain. 
Since it is a density, it must also satisfy $\int_{\R^d}p=1$.
Therefore, we conjecture that Assumption~\eqref{simplifyingAssumption} can only be violated on very few parts of the domain.
